PIQUE: Progressive Integrated QUery Operator with Pay-As-You-Go Enrichment

Big data today in the form of text, images, video, and sensor data needs to be enriched (i.e., annotated with tags) prior to be effectively queried or analyzed. Data enrichment (that, depending upon the application could be compiled code, declarative queries, or expensive machine learning and/or signal processing techniques) often cannot be performed in its entirety as a pre-processing step at the time of data ingestion. Enriching data as a separate offline step after ingestion makes it unavailable for analysis during the period between the ingestion and enrichment. To bridge such a gap, this paper explores a novel approach that supports progressive data enrichment during query processing in order to support interactive exploratory analysis. Our approach is based on integrating an operator, entitled PIQUE, to support a prioritized execution of the enrichment functions during query processing. Query processing with the PIQUE operator significantly outperforms the baselines in terms of rate at which answer quality improves during query processing.

==> AnswerSetSelection.tex <==
\section{Answer Set Selection}
\label{sect:Threshold}

In this section, we will explain our strategy of choosing a subset of the objects from $D$ that must be returned as part of the answer set. This strategy is based on choosing an answer set that will maximize the expected quality (in terms of $F_1$ measure) of the answer set. 

% Given the set of objects with their associated probabilities \hl{Remember that we have to talk always about the multifeature scenario! associated probabilities per feature? how do we go from the probabilities from multiple features to a single one? all of this has to be explained before or nobody will understand this section.}
For every object we assign a probability value first for this phase. The probability value used in this case is the $joint \ \ probability$ value $P_{i.}$, as it represents the probability of the object containing all the $n$ features together. Based on this value, we choose a subset of objects from $D$ which will maximize the expected $F_1$ measure of the answer set. For doing this, first we try to establish a relationship between the $joint \ \ probability$ of the objects in $D$ and the quality of an answer set $A$ chosen from $D$  . 

\begin{comment}
We associate a probability value with each objects in the dataset which represents the probability of the object containing the features mentioned in the query. If a query contains single predicate then we use the probability of that feature as the probability of the object. On the other hand, the query may contain multiple features. In that scenario, each object will have more than one probability value corresponding to each features. Suppose a query has two predicates on feature $f_1$ and $f_2$, then every objects will have two probabilities $p_1$ and $p_2$ associated with it. Since the query is a conjunctive query and we assume that the features are independent of each other, then probability that the object has both feature $f_1$ and $f_2$ is $p_1p_2$. We refer this probability value as the probability of an object for multi-feature scenario. Now we will describe our strategy of selecting an answer set using these object probability values.
We first sort the objects based on their probability values. Then, starting from the object with the highest probability, we check whether adding such an object to the answer set will increase the expected F-1 measure of the answer or not. The moment that adding an object to the answer set decreases the F-1 measure, we stop checking the rest of the object. A subset of objects $A$ chosen from $D$, will have maximum expected quality, if the following strategy is used for choosing $A$: objects must be included in answer set starting from $p_1$ until the point expected quality of the answer set drops. 
\end{comment}

\begin{theorem}\label{theorem:threshold}
Suppose joint probability values of objects in $D$ are as follows: \textit{p\textsubscript{1},p\textsubscript{2},p\textsubscript{3},p\textsubscript{4}... p\textsubscript{n}} where the probability values are sorted in descending order, i.e. \textit{p\textsubscript{1} $\geq$ p\textsubscript{2} $\geq$ p\textsubscript{3} $\geq$ ...$\geq$ p\textsubscript{n} }. A subset of objects $A$ chosen from $D$, will have maximum expected quality, if $A$ = \{$o_i$ $\vert$ $p_i > p_{\tau}$ \} where $p_{\tau}$ is the probability for which expected quality of the answer set drops for the first time. We call this probability value $p_\tau$ as $threshold$ probability.
\end{theorem} 

%\begin{proof}
In order to prove this theorem, we first show that if we keep adding objects in the answer set starting from highest probability $p_1$, then quality of the answer set will monotonically increase. After this, we show that if the $F_1$ measure decreases for the first time at a particular point, then there is no need to include those objects in the answer set, i.e., the quality of the answer set will keep decreasing.Remainder of the proof of this theorem can be found in Appendix \ref{appendix:proofs}.

\medskip


\textbf{Threshold as a function of individual probabilities:} \label{ref:ThresholdFunction}
In this section we will define the threshold value in terms of probability values of the objects inside the answer set. As we have seen in section \ref{theorem:threshold}, $F_1$ measure will monotonically increase up to a certain probability $p_m$ and then it will keep decreasing monotonically. So the answer set will contain all the objects whose probability value is more than $p_m$. Lets denote $F_i$ as the $F_1$ measure of the answer set if we include $i-th$ object and $F_{i+1}$ be the $F_1$ measure, if we include $(i+1)-th $ object in the answer set.  

\begin{equation}
\begin{split}
\Delta(F_1) &= \frac{p_1+p_2+...p_{m+1}}{m+1+k} - \frac{p_1+p_2+...p_m}{m+k} , where,  k = \sum\limits_{i=1}^N p_i \\
&= \frac{\splitfrac{(m+k)(p_1+p_2+...+p_{m+1})}{-(p_1+p_2+...+p_m)(m+1+k)}}{(m+1+k)(m+k)} \\
&=  \frac{\splitfrac{(m+k)(p_1+p_2+...+p_{m}) + (m+k)p_{m+1}}{-(p_1+p_2+...+p_m)(m+k) - (p_1+p_2+...+p_m)}}{(m+1+k)(m+k)} \\
&= \frac{p_{m+1}(m+k) - (p_1+p_2+...p_m)}{(m+1+k)(m+k)}
\end{split}
\end{equation}

$F_1$ measure will keep increasing as long as the value of function $\Delta(F_1)$ remains positive. Thus the threshold value will be the lowest value of $m$ for which $\Delta(F_1)$ value becomes negative for the first time:

\begin{equation}\label{eqn:DeltaThreshold}
\begin{split}
\Delta(F_1) < 0 & \Rightarrow p_{m+1}(m+k) - (p_1+p_2+...p_m) < 0 \\
& \Rightarrow p_{m+1}(m+k) < (p_1+p_2+...p_m) \\
& \Rightarrow p_{m+1} < \frac{(p_1+p_2+...p_m)}{(m+k)}
\end{split}
\end{equation}
So an object with probability $p_m$ will be a threshold probability if the following two inequalities hold: 
\begin{equation}\label{eqn:ThresholdInequalityGreater}
\begin{split}
 p_{m} > \frac{(p_1+p_2+...p_{m-1})}{(m-1+k)} ,and
\end{split}
\end{equation}
\begin{equation}\label{eqn:ThresholdInequalityLess}
p_{m+1} < \frac{(p_1+p_2+...p_m)}{(m+k)}
\end{equation}

Based on the above theorem and equations \ref{eqn:ThresholdInequalityGreater} and \ref{eqn:ThresholdInequalityLess}, we can conclude that the threshold has to be recomputed every time probability of any object changes in the dataset $D$. In the next subsection we show how can we reduce the number of threshold re-computation. First we derive a relationship between change in probability of an object and the current threshold value. 

\textbf{Change in threshold value with the change in probability value:}
In this section, we consider how threshold values get affected as a result of change in probabilities in the answer set. First, we will consider probability change of an object which is already in the answer set and then we will consider an object which is currently not in the answer set. In the first scenario, for an object $o_i$, already in answer set, there can be three possibilities:
\begin{itemize}
  \item new probability of the object increased from the current probability 
  \item new probability of the object decreased from the current probability but new probability is still above the current threshold
  \item the probability of the object decreased from the current probability and it went below the current threshold
\end{itemize}  

In the first sceanrio, where the probability of object increases from the current probability, then threshold of the answer set can increase based on the amount of change in probability value.
\begin{definition}
If probability value of an object $o_i$ inside the answer set increases then the threshold can remain same or it can increase i.e. some trailing objects might move out of the answer set. Threshold value will increase when the change in probability value $\Delta > \frac{p_{m+1}(m+k) - \sum\limits_{i=1}^{m}p_i}{1-p_{m+1}}$, otherwise the threshold will remain same.
\end{definition}

\begin{proof}
Lets assume that probability of object $o_i$ is increased from $p_i$ to $p_i + \Delta$. Now if we consider that initially object $o_{m+1}$ is the threshold, then the following inequality holds:
\begin{equation}\label{ref:p_(m+1)}
\begin{split}
&p_{m+1} > \frac{(p_1+p_2+...p_m)}{(m+k)} \\
&\Rightarrow p_{m+1}(m+k) > (p_1+p_2+...p_m)
\end{split}
\end{equation}

Now if we consider that $o_{m+1}$ is still the threshold even after increasing the probability of object $o_i$ then the following inequality must hold:
\begin{equation}\label{eqn:deltaP}
\begin{split}
&p_{m+1} > \frac{(p_1+p_2+..+p_i+\Delta+....p_m)}{(m+k+\Delta)} , where,  k = \sum\limits_{j=1}^N p_j \\
&\Rightarrow p_{m+1}(m+k+\Delta) > (p_1+p_2+..+p_i+\Delta+....p_m) \\
&\Rightarrow p_{m+1}(m+k) + \Delta p_{m+1} > p_1+p_2+...+p_m + \Delta \\
&\Rightarrow p_{m+1}(m+k) - (p_1+p_2+...+p_m) > \Delta (1-p_{m+1})
\end{split}
\end{equation}

From equation \ref{ref:p_(m+1)}, we get that $p_{m+1}(m+k) - (p_1+p_2+...+p_m) >0$. So equation \ref{eqn:deltaP} will be as follows:
\begin{equation}
\begin{split}
& \Delta (1-p_{m+1}) < p_{m+1}(m+k) - (p_1+p_2+...+p_m) \\
&\Rightarrow\Delta < \frac{p_{m+1}(m+k) - (p_1+p_2+...+p_m)}{1-p_{m+1}}
\end{split}
\end{equation}
So threshold value will remain constant as long as $\Delta$ value is less than $\frac{p_{m+1}(m+k) - \sum\limits_{i=1}^{m}p_i}{1-p_{m+1}}$, otherwise it will be increased.

\end{proof}

\begin{definition}
If probability value of an object $o_i$ inside the answer set gets reduced but it still stays above the current threshold probability, then the threshold will either remain same or it will decrease. This implies that the objects which were already in the answer set will always remain in the answer set, whereas some new objects might get added in the answer set.
\end{definition}
Suppose the probability of object $o_i$ gets decreased from $p_i$ to $p_i- \Delta$ . According to the inequality \ref{eqn:ThresholdInequalityGreater}, if object $o_m$ is still in the answer set, then the following condition must hold:
\begin{equation}
\begin{split}
p_{m} > \frac{(p_1+p_2+...p_{m-1} - \Delta)}{(m-1+k - \Delta)}
\end{split}
\end{equation}
Now since the right side of the above inequality $\frac{(p_1+p_2+...p_{m-1} - \Delta)}{(m-1+k - \Delta)}$ is reduced from the previous value, i.e. $\frac{(p_1+p_2+...p_{m-1})}{(m-1+k)}$, this inequality will always hold. Furthermore if the  inequality \ref{eqn:ThresholdInequalityLess} also holds, then the previous threshold will remain same, otherwise more objects will be included in the answer set.


\begin{definition}
If probability value of an object $o_i$ inside the answer set gets reduced and it goes below he current threshold probability, then the threshold might increase or decrease. The threshold increases when the change in probability value $\Delta > \frac{p_i}{p_m} -1$, where $p_m$ is the probability value of the last object in the answer set. The threshold value decreases when the change in probability value $\Delta < \frac{p_i}{p_{m+1}}-1$
\end{definition}

Lets consider that, the probability of object $o_i$ reduced from $p_i$ to $p_i-\Delta$. The new probability $p_i -\Delta$ is lower than the current threshold probability. Suppose object with probability $p_m$ was inside the answer set which implies that $p_m$ was greater than $\frac{(p_1+p_2+...p_{m-1})}{(m-1+k)}$ according to inequality \ref{eqn:ThresholdInequalityGreater}. Let us denote the numerator by $X$ and the denominator by $Y$. Now since the object $o_i$ moved out of the answer set, the new numerator will be $X-p_i$ and new denominator will be $Y-1-\Delta$. So the new value in the right hand side of inequality \ref{eqn:ThresholdInequalityGreater} becomes $\frac{X-p_i}{Y-1-\Delta}$. If the value $\frac{X-p_i}{Y-1-\Delta}$ becomes greater than $\frac{X}{Y}$, then the inequality \ref{eqn:ThresholdInequalityGreater} will not hold and threshold value will be increased. This condition arises when $\Delta$ value is more than $\frac{p_i}{p_m} -1$. Note that $\frac{p_i}{p_m}$ is more than 1, since $p_i>p_m$ as object with probability $p_m$ was the last object in the answer set.  


Lets consider \ref{eqn:ThresholdInequalityLess} for this scenario, which implies that object $o_{m+1}$ with probability $p_{m+1}$ was not in the answer set. According to \ref{eqn:ThresholdInequalityLess}, $p_{m+1}$ was less than $\frac{(p_1+p_2+...p_m)}{(m+k)}$. Now the right hand side of inequality \ref{eqn:ThresholdInequalityLess} becomes $\frac{(p_1+p_2+...p_m)-p_i}{(m+k) -1-\Delta}$. Lets denote the numerator as $X-p_i$ and denominator as $Y-1-\Delta$. So if the value of $\frac{X-p_i}{Y-1-\Delta}$ becomes smaller than previous value of $\frac{X}{Y}$, then the threshold value will be decreased. This condition will arise when $\Delta < \frac{p_i}{p_{m+1}} -1$

\textbf{Scenario 2:} Lets consider objects which were not in the answer set. For this scenario there can be three possibilities:
\begin{itemize}
  \item the probability of the object increased and it became more than the current threshold probability.
  \item the probability of the object increased but the new probability is less than current threshold probability
  \item the probability of the object decreased 
\end{itemize}  

\begin{definition}
If probability value of an object outside of answer set, increases and it becomes more than current threshold then the current threshold might get increased, i.e. some objects which were earlier in the answer set, might move out of the answer set.
\end{definition}
\begin{proof}
Suppose $o_m$ was the last object in the answer set, which implies that $p_m$ was greater than $\frac{(p_1+p_2+...p_{m-1})}{(m-1+k)}$, according to inequality \ref{eqn:ThresholdInequalityGreater}. Lets denote this fraction by $\frac{X}{Y}$.Now the right hand side of inequality \ref{eqn:ThresholdInequalityGreater} will be updated to $\frac{X+p_k}{Y+1+\Delta}$. If this new value is more than previous value of $\frac{X}{Y}$, and $p_m$ is less than this new value, then object $o_m$ will be moved out of answer set.
\end{proof}

\begin{definition}
If probability value of an object outside of answer set, increases but it does not go above the current threshold, then the current threshold value remains same.  
\end{definition}

\begin{proof}
Suppose $o_m$ was the last object in the answer set. So probability $p_m$ was greater than $\frac{(p_1+p_2+...p_{m-1})}{(m-1+k)}$, according to inequality \ref{eqn:ThresholdInequalityGreater}.Lets denote it by $\frac{X}{Y}$. Suppose the object we are referring to is $o_k$ which was not in the answer set and probability value of this object got increased from $p_k$ to $p_k+\Delta$ In the new right hand side of inequality \ref{eqn:ThresholdInequalityGreater}, numerator stays same, as no extra object was added in the answer set, denominator gets increased from $Y$ to $Y+\Delta$. So the new right hand side $\frac{X}{Y+\Delta}$ gets smaller than previous right hand side $\frac{X}{Y}$, which implies that object $o_m$ will remain in the answer set.
\end{proof}

Based on above observations, given $k$ objects whose probability changes, an optimal incremental update algorithm to determine answer set can be devised. 



==> Extra.tex <==
\begin{table}[t]\label{QueryTable}
\small
\centering
\begin{center}
 \begin{tabular}{|c|c|} 
 \hline
 \textbf{Id} & \textbf{Query} \\
 \hline
 $Q1$ & $< {\tt G = Male} \: \Lambda \: {\tt Precise_1 = P_1} \: \Lambda \: \cdots$ \\ 
 & $\: \Lambda \: {\tt Precise_5 = P_n}>$ \\ 
 \hline
 $Q2$ & $<{\tt S  = Positive} \:\:\: \Lambda \:\:\: {\tt Precise_1 == P_1} \: \Lambda \: \cdots \: $\\
 & $\Lambda \:\:\: {\tt Precise_n = P_n}>$\\
 \hline
 $Q3$ & $<{\tt G = Male} \: \Lambda \: {\tt Ex = Smile} \: \Lambda \: {\tt Precise_1 = P_1} \: \Lambda \: \cdots \: $ \\
 &$\Lambda \: {\tt Precise_n = P_n} >$\\
 \hline
 $Q4$  & $<{\tt G = Male} \: \Lambda  \: {\tt A = 30}  \: \Lambda \: {\tt Precise_1 = P_1} \: \Lambda \: \cdots $ \\
 &$ \: \Lambda \: {\tt Precise_n = P_n} $ \\
 \hline
 $Q5$ & $<{\tt G = Male} \: \Lambda \: {\tt Ex = Smile} \: \Lambda \: {\tt A = 30} \: \Lambda \:  $ \\
 &${\tt Precise_1 = P_1}  \: \Lambda \:  \cdots \: \Lambda \: {\tt Precise_n = P_n}>$ \\
 \hline
\end{tabular}
\vspace{-0.15cm}
\caption{Queries used.}\label{QueryTable}
%\vspace{-0.3cm}
\label{table:Query}
\end{center}
\end{table}

For clarity, we will present the paper as if none of tagging functions were run on any objects prior to the arrival of the query. In Section~\ref{sect:experiments}, we discuss how our approach deals with the case where the outputs of the tagging functions run in previous queries are cached and study the impact of different levels of caching on the performance of the approach.


\begin{itemize}
\item We propose a progressive approach to data enrichment and query evaluation entitled PIQUE that quantizes time into epochs and adaptively enr 
   
\item We present an algorithm for the problem of generating an execution plan that has the highest potential of improving the quality of the answer set in the corresponding epoch.
       
\item We present an efficient strategy to estimate the benefits of the possible triples (i.e., object-predicate-function triple) \yat{ rest should be removed} based on different properties (i.e., output of previous functions, cost and quality of remaining functions).    
    
\item We experimentally evaluated PIQUE in different domains (i.e., images and tweets) using real datasets and tagging functions and demonstrate the efficiency of our solution.
\end{itemize}




Join Query Extension:

\vspace{0.1cm}
\noindent
\textbf{Join Queries.} In this section, we explain in details how PIQUE deals with queries containing join operators where the join condition is on imprecise attribute. Let us consider an example query containing join operators where the join conditions are on imprecise attributes as shown in Figure \ref{fig:joinQueryExample} left. In this query all the attributes $a$, $b$ and $c$ are imprecise attributes. PIQUE rewrites the query by placing decision nodes (denoted by $\epsilon$) in the query tree as shown in Figure \ref{fig:joinQueryExample} right. The possible decisions that are made by PIQUE for a block are as follows: \textit{Enrich Now} or \textit{Evaluate Now}. 

At any point of time, PIQUE determines if the objects inside a given block should be enriched further. Once an \textit{Enrich Now} decision is made for a certain block, PIQUE enriches all the objects inside the block. For each objects inside the block, it performs the triple generation step (Section \ref{triple generation}) and execute all the generated triples from the block. The process of making the decision is performed by exploring a tradeoff between the benefit of enrichment and the benefit of query evaluation. For example, for a given operator, say (R $\bowtie$ S), if a certain block $R_1$ of $R$ contains objects with very high joint probability value, then most likely it will join with a large number of objects from relation $S$ and will subsequently produce large number of tuples in the answer set of the query. In this scenario, enriching further might not produce that much benefit to the final quality of the answer. In this scenario, PIQUE will make the \textit{Evaluate Now} decision for $R_1$. On the other hand, if enriching a certain block can result in significant improvement of the quality of the answer set from the previous epoch, then \textit{Enrich Now} decision is made for the block. 

%large number of tuples will be part of the answer set from the objects of the block. 

%In that scenario, PIQUE choose to evaluate the query instead of further enriching the objects inside the block.


\begin{figure}[t]
\Tree[.$\bowtie_{R.c = T.c}$ [.$\bowtie_{R.b = S.b}$ [.$\sigma_a$ R ] S ] T ]
\Tree[.$\bowtie_{R.c = T.c}$ [.$\epsilon_c$ [.$\bowtie_{R.b = S.b}$ [.$\epsilon_b$ [.$\sigma_a$ [.$\epsilon_a$ R ] ] ] [.$\epsilon_b$ S ] ] ] [.$\epsilon_c$ T ] ]
\caption{Query Example.}
\label{fig:joinQueryExample}
\end{figure}



In each epoch, we generate an enrichment plan that consists of a number of sub-plans. Each sub-plan consists of a disk block and a query operator that needs to be executed on the disk block. Execution of the sub-block includes reading of the disk block to memory and the execution of the query operator on the objects of the disk block. In this example, for a certain block of $R$, say $R_1$, PIQUE checks if the block satisfies the selection condition. If it satisfies, then the block is sent to the R $\bowtie$ S operator. PIQUE generates the next subplan, where it evaluates the join condition on block $R_1$ with one of the block of S (say $S_4$). If the block pair satisfies the join condition of $(R.b = S.b)$, then it is passed on to the next query operator R $\bowtie$ S $\bowtie$ T operator. In the next subplan, PIQUE reads one block of $T$ (say $T_6$) and checks the join condition of ($R.c = T.c$) with the previously outputted block pair of $\langle R_1, S_4 \rangle$. If the block triple $\langle R_1, S_4, T_6 \rangle$ satisfies the final join condition, then PIQUE performs the threshold selection algorithm on the composite objects formed using the objects of blocks $R_1$, $S_4$ and $T_6$ and outputs the objects in $\mathsf CS_w$ to the answer set. In the following we explain how PIQUE chooses the blocks from each relations based on the query evaluation benefit value.

%We maintain a single priority queue containing all the blocks of $R$, $S$ and $T$ and denote it as BlockPQ. Each blocks in the priority  







%\dg{previous paragraph} Finally,  PIQUE as described is restricted to join conditions over precise attributes\footnote{In our experience of using PIQUE in the context of a sensor-driven smart environment at UCI \cite{tippers}, such queries are the predominant use cases.}. Extending PIQUE to support join conditions over imprecise attributes (e.g., $R \bowtie_{R.a = S.a} S $, where $a$ is an imprecise attribute of $R$ and $S$) requires significant extension, similar in nature to join evaluation on probabilistic databases~\cite{Dalvi_2007}. In particular, instead of creating triples on objects, we consider triples over the join output of objects (i.e.,  for $R \bowtie_{R.a = S.a} S $, PIQUE will consider each joined composite object $\langle o_i, o_j\rangle$, where $o_i \in R$ and $o_j \in S$, as a candidate object and create triples for it). The potential quadratic overhead of such a technique can be overcome by creating appropriate blocks and using block-level enrichment plans. We discuss such a strategy in the extended version of the paper \cite{ExtendedPaper}. 

%To reduce overhead, instead of creating triples for all pairs, join predicates are evaluated in units of blocks instead of objects during each epoch.  where $a$ is an imprecise attribute of $R$ and $S$) as follows. We enrich the join attribute $a$ on both datasets present in the join query. We treat each possible pair of the cartesian product (i.e., $ R \times S)$ as an object and create a set of blocks from such objects. To reduce the complexity of this extension, join predicates are evaluated in each epoch in units of blocks instead of objects. A detailed description of this extension can be found~\cite{ExtendedPaper}.

%Finally, we have restricted the above discussion to join queries in which the join conditions are over precise attributes\footnote{In our experience of using PIQUE in the context of a sensor-driven smart environment at UCI \cite{tippers}, such queries are the predominant use cases.}. PIQUE can be extended to deal with join queries over imprecise attributes (e.g., $R \bowtie_{R.a = S.a} S $, where $a$ is an imprecise attribute of $R$ and $S$) as follows. We enrich the join attribute $a$ on both the datasets present in the join query. We each possible pair present in the cartesian product (i.e., $ R \times S)$ and consider it as an object. We create a set of blocks from the objects in the dataset R and S. To reduce the complexity of our approach, we generate a plan on top of these blocks in each epoch.  Details about the extension can be found in the full version of the paper \cite{ExtendedPaper}.



%%%%%%% AQP writeup in the Introduction %%%%%%%

\dg{newly added. need review.} 
The goal of approximate query processing system (AQP) is to provide an approximate answer to aggregation queries with a quality and/or a cost bound \cite{BlinkDB,VerdictDB}. These systems create and maintain a set of beneficial samples based on a previous query workload. Given an aggregation query, the objective of an AQP system translates down to choosing a set of samples for the execution of the query that minimizes the total execution cost while maintaining a certain bound on the quality. AQP design criterias include appropriate sample maintenance both in terms of column sets selection and sample size selection and accurate estimation of error and latency profiles of the samples for a given query. Such approaches are fundamentally different from our approach as the objective in AQP is to reduce the overall cost of query execution while maintaining a certain amount of quality of the answer whereas our objective is to achieve high quality answer as quickly as possible during the query execution. Furthermore, the queries considered in AQP systems are only limited to aggregation queries whereas our approach considers quality improvement for set-based queries.

\begin{comment}
% AQP extra writeup

 The AQP systems provide two types of parameters for the end-users to choose: cost based parameter and accuracy based parameter. In the cost based parameter a user specifies a maximum cost (in terms of time \cite{BlinkDB} or in terms of total disk I/O \cite{verdictDB}) and the system makes sure that the answer achieves the maximum quality that can be achieved within that time interval. In the accuracy-based parameter, a user specifies a quality bound by specifying the appropriate error bound and confidence interval and the system makes sure that the specified quality is achieved in minimum amount of cost. 
\end{comment}



%Proof of benefit ordering theorem:
% This is the part in the beginning
\begin{comment}
 For simplicity of notation, we denote the threshold $\mathcal P^\tau_{w-1}$ of epoch $w-1$ as $\mathcal P_\tau$ in this proof. $E(F_\alpha(\mathsf{A}_{w-1}))$ can be simplified as follows: $\frac{(1+\alpha)(\mathcal P_1+ \cdots +\mathcal P_\tau)}{\alpha(\mathcal P_1+\mathcal P_2+ \cdots +\mathcal P_{|O|})+ \tau}$. We denote the numerator by $X$ and the value of $\alpha(\mathcal P_1+\mathcal P_2...\mathcal P_{|O|})$ in the denominator as $Y$. We denote the value of $\frac{\mathcal P_k}{c^l_n}$ by $\nu_k$ and the value of $\frac{\mathcal P_q}{c^s_v}$ by $\nu_q$. Since $m_1$ objects of $\mathsf{A}_{w-1}$ move out of $\mathsf{A}_{w}$ as a result of changing the joint probability value of $o_k$ from $\mathcal P_k$ to $\hat{\mathcal P}_k$, the $E(F_\alpha)$ measure of the answer set in epoch $w$ due to the execution of the triple ($o_k$, $R^l_m$, $f^l_n$) is as follows:
\begin{equation}
\vspace{-0.1cm}
F_{\alpha k}= \frac{\splitfrac{X-(1+\alpha)\cdot(\mathcal P_\tau+\mathcal P_{\tau-1}+...\mathcal P_{\tau-(m_1-1)})}{+(1+\alpha)\cdot(\mathcal P_k+\Delta \mathcal P_k)}}{Y+(\tau-m_1) + \alpha \cdot \Delta{\mathcal P_k}}
\end{equation}

%\splitfrac{(\tau+k)(\mathcal P_1+\mathcal P_2+...+\mathcal P_{\tau+1})}{-(\mathcal P_1+\mathcal P_2+...+\mathcal P_\tau)(\tau+1+k)}
 Similarly for triple ($o_q$, $R^s_t$, $f^s_v$), $m_2$ objects which were part of $\mathsf{A}_{w-1}$, move out of $\mathsf{A}_{w}$ as a result of changing the joint probability value of $o_q$ from $\mathcal P_q$ to $\hat{\mathcal P}_q$. The $E(F_\alpha)$ measure of the answer set in epoch $w$ will be as follows:
 \vspace{-0.1cm}
 \begin{equation}
 \vspace{-0.2cm}
 F_{\alpha q} = \frac{\splitfrac{X-(1+\alpha)\cdot(\mathcal P_\tau+\mathcal P_{\tau-1}+...\mathcal P_{\tau-(m_2-1)})+}{(1+\alpha)\cdot(\mathcal P_q+\Delta \mathcal P_q)}}{Y+(\tau-m_2) + \alpha \cdot \Delta{\mathcal P_q}}
\end{equation}

\end{comment}




%%%%%%%%%%% Relative Benefit ordering theorem proof (complete proof) %%%%%%% 
\textbf{Proof Sketch.} We prove this theorem as follows: given three possible cases of $m_1$ and $m_2$, we consider all possible combinations (16 possible combinations) of the values of $\mathcal P_k$, $\mathcal P_q$, $\Delta \mathcal P_k$, and $\Delta \mathcal P_q$ and show if Equation \ref{eqn:DeriveBenefitCondition3} holds, then the benefit of $(o_k, R^i_l, f^i_m)$ will be higher than the benefit of $(o_q, R^s_t, f^s_v)$. In the following we provide the proof of three such scenarios:

 For ease of notation, we denote the threshold $\mathcal P^\tau_{w-1}$ of epoch $w-1$ as $\mathcal P_\tau$ in this proof. The notation of $E(F_\alpha(\mathsf{A}_{w-1}))$, i.e., $\frac{(1+\alpha)(\mathcal P_1+ \cdots +\mathcal P_\tau)}{\alpha(\mathcal P_1+\mathcal P_2+ \cdots +\mathcal P_{|O|})+ \tau}$ can be simplified as $\frac{X}{Y+ \tau}$. We denote the value of $\frac{\mathcal P_k}{c^l_n}$ by $\nu_k$ and the value of $\frac{\mathcal P_q}{c^s_v}$ by $\nu_q$. Rewriting the expression of benefit for both the triples, the benefit value of triple ($o_k$, $R^l_m$, $f^l_n$) will be higher than the triple ($o_q$, $R^s_t$, $f^s_v$), when the following condition holds:

The benefit value of triple ($o_k$, $R^l_m$, $f^l_n$) will be higher than the triple ($o_q$, $R^s_t$, $f^s_v$), when the following condition holds: %$\nu_{k}F_{\alpha k} > \nu_{q}F_{\alpha q}$. 
\begin{equation}\label{pm_upperbound}
\begin{split}
&\nu_k(\frac{\splitfrac{X-(1+\alpha)\cdot(\mathcal P_\tau+\mathcal P_{\tau-1}+...\mathcal P_{\tau-(m_1-1)})+}{(1+\alpha)\cdot(\mathcal P_k+\Delta \mathcal P_k)}}{Y+(\tau-m_1) + \alpha\cdot\Delta{\mathcal P_k}}) > \\
&\nu_q(\frac{\splitfrac{X-(1+\alpha)\cdot(\mathcal P_\tau+\mathcal P_{\tau-1}+...\mathcal P_{\tau-(m_2-1)})+}{(1+\alpha)\cdot(\mathcal P_q+\Delta \mathcal P_q)}}{Y+(\tau-m_2) + \alpha\cdot\Delta{\mathcal P_q}}) 
\end{split}
\end{equation}


%We consider the different cases of $\Delta \mathcal P_k$, $\Delta \mathcal P_q$, $(\mathcal P_k + \Delta \mathcal P_k)$, and $(\mathcal P_q + \Delta \mathcal P_q)$ values and establish the conditions in which Equation \ref{pm_upperbound} is satisfied.



\vspace{0.1cm}
\noindent
\textbf{Case 1: $\Delta \mathcal P_k$ $<$ $\Delta \mathcal P_q$, $\mathcal P_k + \Delta \mathcal P_k$ $>$ $\mathcal P_q + \Delta \mathcal P_q$,  and $m_1 > m_2$}. %\dg{newly added} 

Comparing both the denominators of Equation \ref{pm_upperbound}, we can see that $(\tau-m_1)<(\tau-m_2)$ and $\Delta \mathcal P_k$ $<$ $\Delta \mathcal P_q$. This implies that the denominator on the L.H.S. is smaller than the denominator on the R.H.S. In the numerator of L.H.S, the value of $(\mathcal P_\tau+\mathcal P_{\tau-1}+...\mathcal P_{\tau-(m_1-1)})$ is higher than $(\mathcal P_\tau+\mathcal P_{\tau-1}+...\mathcal P_{\tau-(m_2-1)})$ as $m_1$ is higher than $m_2$. Furthermore, if $\nu_k(\mathcal P_k +\Delta \mathcal P_k) > \nu_q(\mathcal P_q+ \Delta \mathcal P_q)$ then the numerator of the L.H.S. will always be higher than the numerator of the R.H.S. Thus we can conclude that the Equation \ref{pm_upperbound} will be satisfied when the condition $\nu_k(\mathcal P_k+\Delta \mathcal P_k) > \nu_q(\mathcal P_q+ \Delta \mathcal P_q)$ is satisfied. 


%\dg{newly added} 

\vspace{0.1cm}
\noindent
\textbf{Case 2: $\Delta \mathcal P_k$ $>$ $\Delta \mathcal P_q$, $\mathcal P_k + \Delta \mathcal P_k$ $>$ $\mathcal P_q + \Delta \mathcal P_q$, and $m_1 > m_2$}. In Equation \ref{pm_upperbound}, the value of $(\mathcal P_\tau+\mathcal P_{\tau-1}+...\mathcal P_{\tau-(m_1-1)})$ on the L.H.S is higher than $(\mathcal P_\tau+\mathcal P_{\tau-1}+...\mathcal P_{\tau-(m_2-1)})$ as $m_1$ is higher than $m_2$. In the denominator, although the value of $\Delta \mathcal P_k$ is higher than $\Delta \mathcal P_q$, the total value of $(\tau-m_1 + \alpha \cdot \Delta \mathcal P_k) $ will be lower than $ (\tau-m_2 + \alpha \cdot \Delta \mathcal P_q)$ as both $\Delta \mathcal P_k$ and $\Delta \mathcal P_q$ are less than one.

\begin{comment}
 
\vspace{0.1cm}
\noindent
\textbf{Case 3: $\Delta \mathcal P_k$ $<$ $\Delta \mathcal P_q$, $\mathcal P_k + \Delta \mathcal P_k$ $>$ $\mathcal P_q + \Delta \mathcal P_q$ and $m_1,m_2=0$}.%\dg{newly added}
Substituting $m_1 = 0 $ and $m_2 = 0$ in Equation \ref{pm_upperbound}, we get the following equation:
\begin{equation}\label{pm_upperbound_const_thr}
\begin{split}
\nu_k &( \frac{X+(1+\alpha)\cdot(\mathcal P_k+\Delta \mathcal P_k)}{Y+ \tau + \alpha \cdot\Delta{\mathcal P_k}}) >\\ 
&\nu_q ( \frac{X+(1+\alpha)\cdot(\mathcal P_q+\Delta \mathcal P_q)}{Y+ \tau + \alpha \cdot\Delta{\mathcal P_q}} )
\end{split}
\end{equation}


The denominator of L.H.S. is lower than the denominator of R.H.S. as $\Delta{\mathcal P_k} < \Delta{\mathcal P_q}$. Furthermore, if the condition: $\nu_k(\mathcal P_k+\Delta \mathcal P_k) > \nu_q(\mathcal P_q+ \Delta \mathcal P_q)$ is satisfied, then the numerator of the L.H.S. will be higher than the R.H.S. This implies that the L.H.S will always be higher than the R.H.S., if the condition $\nu_k(\mathcal P_k+\Delta \mathcal P_k) > \nu_q(\mathcal P_q+ \Delta \mathcal P_q)$ is satisfied.


\end{comment}


\begin{comment}
Removed this part.
\noindent The possible values of $m_1$ and $m_2$ are as follows: 
\begin{itemize}[leftmargin=*]
\item  $m_1 = m_2 = 0$. This scenario implies that the threshold probability value $\mathcal P^{i}_\tau$ did not change given the new estimated joint probability values $\hat{\mathcal P}_k$ and $\hat{\mathcal P}_q$. 
\item $m_1 > m_2$, $m_1> 0$, and $m_2> 0$. This scenario implies that the threshold probability value $\mathcal P^{i}_\tau$ increased more due to the joint probability $\hat{\mathcal P}_k$ as compared to $\hat{\mathcal P}_q$.
\item  $m_2 > m_1$, $m_1 >0$, and $m_2 > 0$. This scenario implies that the threshold probability value $\mathcal P^{i}_\tau$ increased more due to the joint probability of $\hat{\mathcal P}_q$ as compared to $\hat{\mathcal P}_k$. 
\item $m_1 = m_2$, $m_1> 0$, and $m_2 > 0$. This scenario implies that the threshold probability value $\mathcal P^{i}_\tau$ increased by the same amount due to the probability values $\hat{\mathcal P}_k$ and $\hat{\mathcal P}_q$. 
\end{itemize}

\end{comment}


%%%%% Scenarios in the introduction %%%%%%
PIQUE is motivated by several real-life scenarios; two of which are listed below:
\vspace{0.1cm}
\noindent
{\bf Scenario 1:} Consider a smart building deployment\footnote{This query is based on our experience in creating a smart IoT test bed at Donald Bren Hall of UCI~\cite{tippers}} wherein a diverse set of sensors are deployed to track the movement of people inside the buildings. Analysis of Wi-Fi signal might provide a cheap (but relatively coarse) localization of the people whereas face detection/recognition over images captured by hundreds of cameras installed within the building may offer an accurate, albeit more expensive, alternative. Exhaustive analysis of continuously captured video is likely computationally infeasible and/or wasteful. Instead, PIQUE answers queries based on subjects' location progressively by performing expensive video analysis on a selective portion of the data that helps in answering the query. 

\vspace{0.1cm}
\noindent
{\bf Scenario 2:} Consider a tweet monitoring system~\cite{tweet_topic_follow_up_demo} that tracks events in real-time over social media. Different tagging functions may be used to determine the tweet topics, the location where the tweet was posted from, references to locations in the text (if any), the sentiment/tone of the tweets, etc. While cheap variants of tagging functions for such enrichment tasks may exist,  tagging functions achieving a high-quality labelling  may incur significant computational costs. A user may be interested in analyzing social media posts (e.g., determining the geographical regions where the sentiment of tweets for a specific topic/event is mostly positive). Such analysis will require executing several tagging functions -- topic determination, location determination, and sentiment detection. PIQUE selectively chooses a set of tweets for each of these enrichment tasks with the goal of progressively answering the query. 


%%% Join query section %%%

 and face recognition~\cite{person_detection}
@inproceedings{Twitter_Sentiment_Dataset,
  title={Twitter Sentiment Classification using Distant Supervision},
  author={Alec Go and Richa Bhayani and Lei Huang},
  year={2009}
}


\vspace{0.1cm}
\noindent
\textbf{Aggregation Queries and Nested Queries.} We note  that aggregation queries can be evaluated by first executing the query using PIQUE and then performing aggregation on the returned result. Since the value of the aggregation returned over epochs will change, mechanisms can be developed to offer confidence intervals on the aggregated output using the query satisfiability probabilities of the objects. Furthermore, nested queries can be supported using PIQUE if they can first be unnested  \cite{QueryUnnesting}. Evaluating queries that cannot be unnested is more complex and is outside the scope of this paper. 




In the plan generation phase, PIQUE performs the following steps (similar to the steps shown in Section \ref{sect:overview}): \textit{candidate set selection}, \textit{make decision}, \textit{generation of triples}, \textit{benefit estimation},  and \textit{triple selection}. The candidate selection step chooses the set of composite objects which are outside of the answer set of the epoch and consider it as the candidate set $\mathsf CS_{w}$. In the \textit{make decision} step, for each objects present in  $\mathsf CS_{w}$, it makes a decision to either choose to enrich the object, or send the object up the query tree to the next operator or ignore the object and keep it at the same level of the query tree. Thus, it can make three decisions: \textit{enrich}, \textit{move up}, and \textit{ignore}. Once the enrichment decision is made, only the composite objects which had \textit{enrichment} decision are kept in $\mathsaf CS_w$ and the remaining objects are eliminated. In the triple generation step of PIQUE, it generates the triples for each of the composite objects present in $\mathsf CS_w$. The \textit{benefit estimation} step measures the relative benefit of the triples generated in the previous step. The \textit{triple selection} step orders them based on their relative benefit value and maintain them in a priority queue. 





%%% General query prev writeup %%%%%%

For each objects of the base relations (i.e., $R$, $S$ and $T$) PIQUE, uses the query satisfiability probability of the object to make the enrichment decision.

An object $o_k$ is considered to be a part of the final answer set of the query if it is part of at-least one object of the final query answer. The QSP value of an object always improves from the leaf node of the query tree to the root node of the tree. When an object is moved up the tree to the next operator, QSP value is updated by measuring the conditional probability of the object to be part of the final answer set given it satisfied an earlier query predicate.



%%Consider that an object $o_i$ has a probability $p_i$ of satisfying all the query predicates. In a certain epoch $w-1$, based on the QSP value of $p_k$, suppose the expected quality of the answer set was $E(F_{\alpha}(\mathsf A_{w-1}))$. After the enrichment of the object, if the QSP value increases, then more number of tuples get generated in the final answer set and the expected quality of the answer increases. We determine the new quality of the answer set and denote it as $E(\hat{F}_{\alpha}(\mathsf A_{w-1}))$. Based on these two values we calculate the benefit of enrichment of the object by measuring the improvement of the quality of the answer per unit cost.




%PIQUE rewrites the query by placing decision nodes (denoted by $\epsilon$) in the query tree as shown in Figure \ref{fig:joinQueryExample} right. 

%If an operator is a selection operator in the query tree, PIQUE always pushes the block up the query tree to the next operator as long as there exists at-least one object inside the block that has non-zero probability of satisfying the selection predicate. If an operator is a join operator, then two blocks (or composite blocks) satisfy the join condition, iff there exists at-least one objects (or composite objects) from both the inputs that satisfy the join condition. 




%The decision nodes are placed before each operators in the query tree that contains an imprecise attribute. The possible decisions that can be made by these operators are as follows: \textit{Enrich Now} or \textit{Pass to Next}. 

%The possible decision nodes are denoted by $\epsilon_{a}$, $\epsilon_b$ and $\epsilon_c$ to denote the imprecise attributes of $a$, $b$ and $c$.
%\item $(\mathcal P_1+\mathcal P_2+\dots \mathcal P_{\tau-1})$

\begin{figure}[t]
\small
\begin{subfigure}[t]{0.15\textwidth}
\vspace{1.5cm}
\Tree[.$\bowtie_{R.a = S.a}$ R S ]
\vspace{1.7cm}
\caption{Query 1.}\label{fig-a}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.15\textwidth}
\Tree[.$\bowtie_{R.c = T.c}$ [.$\bowtie_{R.b = S.b}$ [.$\sigma_a$ R ] S ] T ]
\vspace{2cm}
\caption{Query 2.}\label{fig-b}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.15\textwidth}
\Tree[.$\bowtie_{R.c = T.c}$ [.$\epsilon_c$ [.$\bowtie_{R.b = S.b}$ [.$\epsilon_b$ [.$\sigma_a$ [.$\epsilon_a$ R ] ] ] [.$\epsilon_b$ S ] ] ] [.$\epsilon_c$ T ] ]
\caption{Query 2 Modified Plan.}\label{fig-c}
\end{subfigure}
\caption{Query Example.}
\label{fig:joinQueryExample}
\end{figure}

Suppose relations R, S and T contains two objects each and their QSP values are as follows: $r_1(0.9)$ , $r_2(0.4)$, $s_1(0.8)$, $s_2(0.7)$, $t_1(0.9)$ and $t_2(0.6)$. PIQUE performs the threshold selection algorithm on the composite objects $\langle r_i, s_j, t_k \rangle$ and determines the answer set. The composite objects $\langle r_1, s_1, t_1 \rangle$, $\langle r_1, s_1, t_2 \rangle$ and $\langle r_1, s_2, t_1 \rangle$ will be part of the answer set and the remaining five composite objects will be outside of the answer set.
%$\langle r_1, s_2, t_2 \rangle$, $\langle r_2, s_1, t_1 \rangle$, $\langle r_2, s_1, t_2 \rangle$, $\langle r_2, s_2, t_1 \rangle$, $\langle r_2, s_2, t_2 \rangle$


In the plan generation phase, PIQUE performs the following steps (similar to the steps shown in Section \ref{sect:overview}): \textit{candidate set selection}, \textit{make decision}, \textit{generation of triples}, \textit{benefit estimation},  and \textit{triple selection}. The candidate selection step chooses the set of composite objects which are outside of the answer set of the epoch and consider it as the candidate set $\mathsf CS_{w}$. In the \textit{make decision} step, for each objects present in  $\mathsf CS_{w}$, it makes a decision to either choose to enrich the object, or send the object up the query tree to the next operator or ignore the object and keep it at the same level of the query tree. Thus, it can make three decisions: \textit{enrich}, \textit{move up}, and \textit{ignore}. Once the enrichment decision is made, only the composite objects which had \textit{enrichment} decision are kept in $\mathsaf CS_w$ and the remaining objects are eliminated. In the triple generation step of PIQUE, it generates the triples for each of the composite objects present in $\mathsf CS_w$. The \textit{benefit estimation} step measures the relative benefit of the triples generated in the previous step. The \textit{triple selection} step orders them based on their relative benefit value and maintain them in a priority queue. 

%In the \textit{Make Decision} step, PIQUE executes the function as shown in Figure \ref{fig:decision_function}. 

In the \textit{Make Decision} step of an epoch $w$, for a given object $r_i$, PIQUE first determines the number of composite objects in the answer set that contains the object $r_i$. If all the composite objects are inside the answer (i.e., have QSPs higher than $\mathcal P^{\tau}_{w-1}$), then PIQUE ignores object $r_i$. If $r_i$ has large number of objects inside the answer set and very few objects outside of the answer set, then PIQUE chooses to move the object up the query tree and decide to enrich it later. If $r_i$ has only few composite objects inside of the answer set and has a large number of composite objects very close to the threshold, then PIQUE checks the enrichment benefit. Due to the enrichment of $r_1$ at that level, if it can cause a large number of composite objects to be included in the answer set of epoch $w$, then it chooses to perform enrichment. If $r_1$ has few composite objects inside of the answer set and a large number of objects outside of the answer set but are far from the threshold probability, then PIQUE checks if enrichment at that level can help improving the quality of the answer set. After enrichment of the object, if the expected quality of the answer set is supposed to stay the same, then PIQUE chooses to ignore the object.

Such an approach faces  several challenges as listed below:

\begin{itemize}[leftmargin=*]
\vspace{-0.1cm}
\itemsep-0.1em
    \item Accurate estimation of the QSP value of an object at a given level of the query tree: PIQUE assumes that the operators containing different tag types are independent of each other. Thus, it computes the probability as Sharad: explain how.
    \item Accurate estimation of increment of QSP value of an object when an object is pushed up the query tree: . PIQUE scales the QSP value of the object when it is moved up the query tree by a constant scaling factor $\beta$. 
    
    %In ~\cite{ExtendedPaper}, we show that even if certain objects change their QSP values by a constant factor, PIQUE needs to execute the threshold selection algorithm to determine the answer set.
    \item If the number of objects in the base relations are large and the query is arbitrarily complex, then the complexity of the \textit{Make Decision} step can be very high.  In this scenario, PIQUE uses a block based approach where it makes the decision for a block instead of each objects.
\end{itemize}
% In ~\cite{ExtendedPaper}, we provide the details of how we reduce the complexity of the \textit{make-decision} step and maintain the optimality of the candidate selection step.

%at a certain level of the query tree, enrichment of $r_1$ can 


%The objective is if a large number of composite objects contain a certain block, then there is not much advantage in enriching the block more.

\begin{comment}
\begin{algorithm}[t]
\begin{algorithmic}[1]
\scriptsize
\Procedure{MAKE-DECISION}{$o_k$, $op$, $T_j$, $\mathcal P_k, \mathcal P^{\tau}_{w-1}$}
\State $\mathcal P \gets \Call{Calculate-QSP}{o_k, op, T_j}$
\State $\mathcal P^{\tau}_w \gets \Call{Calculate-Threshold}{\mathcal P}$
 \State $enrichBenefit \gets \Call{Calculate-Enrichment-Benefit}{o_k, op, T_j}$
   
\If{$\mathcal P_0 \geq \mathcal P^{\tau}_{w-1}$, $\mathcal P \geq \mathcal P^{\tau}_{w}$}
    \If{$enrichBenefit \geq 0$}
        \State $decision \gets enrich$
    \Else
        \State $decision \gets move \ \ up$
    \EndIf
  %\State \Call{Add-To-Enrichment-Queue}{$R_i$, $enrichmentBenefit$}
\Else
    \If{$\mathcal P_0 < \mathcal P^{\tau}_{w-1}$, $\mathcal P \geq \mathcal P^{\tau}_{w}$}
        \If{$enrichBenefit \geq 0$}
            \State $decision \gets enrich$ //Enrich the object.
            
        \Else
             \State $decision \gets ignore$ //Ignore the object.
        \EndIf
    \Else 
        \State  $decision \gets ignore$
    \EndIf
\EndIf
\State \Return $ decision$    
\EndProcedure
\captionof{figure}{Decision Function}\label{fig:decision_function}
\end{algorithmic}
\end{algorithm}
\end{comment}




%%%%%%%%%%%%%%% Evaluate now vs enrich now extra write up %%%%%%
In each epoch, using the QSP values of the objects in the base relations, PIQUE chooses to perform enrichment on the tuples in the base relations. In the following we explain the process of enrichment plan generation in PIQUE. Given a complex query of Figure \ref{fig-b}, PIQUE first rewrites the query by adding enrichment operators as shown in Figure \ref{fig-c}. In the plan generation phase, PIQUE performs the following steps (similar to the steps shown in Section \ref{sect:overview}): \textit{candidate set selection}, \textit{make-decision}, \textit{generation of triples}, \textit{benefit estimation}, and \textit{triple selection}. In the candidate selection step of an epoch, PIQUE uses the same technique with $\mathcal O(n)$ complexity as the join query execution to determine the threshold of the final answer set of the query.  

In the \textit{make-decision} step, PIQUE makes two types of decisions for any tuple: \textit{enrich now} or \textit{ignore}.

For a general query, as shown in Figure \ref{fig-c}, that contains multiple selection and join conditions, we consider two types of uncertainty of the objects. First type of uncertainty exists in the value of the object, e.g., tuple $r_1$ has an attribute value of $(a= a_1)$ with a probability of 0.8. We call this as value based probability and denote it as $\mathcal V_k$. Suppose for any two predicates $R^i_l$ and $R^i_m$, a certain object $o_k$ has the probability values of $\mathcal V^i_l$ and $\mathcal V^i_m$.

The second type is the uncertainty, whether a tuple will rise to the top of the query tree or not. We call this as selectivity probability and we denote it as $S_i$. Given this two values we measure the QSP value of a tuple as follows:
\begin{equation}
    QSP(t_1, t_2) = s(t_1,t_2) \cdot \mathcal V_1 \cdot \mathcal V_2
\end{equation}

Each time a tuple is sent up the query tree, the selectivity probability value is increased. For $o_k$, if it is moved to the next operator and the selectivity probability value is updated from $s(t_1,t_2)$ to $s'(t_1,t_2)$, then the QSP value of the tuple will be as follows:
\begin{equation}
    QSP(t_1, t_2) = s'(t_1,t_2) \cdot \mathcal V_1 \cdot \mathcal V_2
\end{equation}


Each time a tuple is enriched, the value-based probability is improved. For $o_k$, if it is enriched and the value based probability value is updated from $\mathcal V_1$ to $\mathcal V'_1$, then the QSP value of the tuple will be as follows:
\begin{equation}
QSP(t_1, t_2) = s'(t_1,t_2) \cdot \mathcal V_1' \cdot \mathcal V_2
\end{equation}

To extend our approach to multiple operators, PIQUE makes two types of decisions: \textit{enrich now} or \textit{do not enrich}. When an object reaches to a query predicate, it either satisfies the predicate or do not satisfy the predicate. If for an object, the predicate is not satisfied, then it stays in that level of the query tree. Unlike traditional query processing approach, such an object can not be eliminated because the reason of not satisfying the predicate can be due to uncertainty in the value of the object.


In the candidate selection step, PIQUE needs to determine the QSP values of all the possible pairs of $R$ and $S$ first and then perform the threshold selection algorithm of Section \ref{Answercomputealgorithm} based on their QSP values. However this approach has an $\mathcal O(n^2)$ time complexity. Instead, in PIQUE we devise a novel approach that has $\mathcal O(n)$ time complexity.

==> Introduction_old_vldb_submission.tex <==
%\vspace{1cm}
\section{Introduction}
\label{sect:introduction}
 

Today, organizations have access to potentially limitless information in the form of web data repositories, continuously generated sensory data, social media posts, captured audio/video data, click stream data from web portals, and so on~\cite{OnlineLiveStat}.
Before such data can be analyzed, it first needs to be enriched (i.e., associated with tags) using appropriate machine learning and/or signal processing techniques.
Examples of enrichment include sentiment analysis~\cite{TweetSentimentAnalysis3,TweetSentimentAnalysis2} over social media posts, named entity extraction~\cite{NamedEntity_Extraction1,NamedEntity_Extraction2} in text, face detection~\cite{face_detection_2} and face recognition~\cite{person_detection} in images, and sensor interpretation and fusion~\cite{sensor_fusion_1} over sensory inputs. Functions used to enrich data (which we refer to as {\em tagging functions}) often exhibit a cost vs. quality trade-off where cheaper functions may produce lower quality results whereas more expensive functions may result in improved quality.

While limited data enrichment (e.g., by running cheap tagging functions) at the ingestion time is typically feasible, running a suite of computationally expensive functions to generate the best possible tags may be impossible due to the speed and volume of the incoming data. Enrichment could also be performed as a separate offline step, but such an approach suffers from several shortcomings. If data is large, it may still be computationally infeasible and/or wasteful (if no query uses the enriched data) to run complex tagging functions on all the data. Even powerful search engine companies (with seemingly limitless resources)  
%while they might extract and index semantic concepts, 
do not fully resolve/link entities over the hundreds of billions of web pages that they collect. Furthermore, an offline enrichment approach does not support real-time (or near real-time) analysis since the data remains unavailable until it is enriched/tagged. Finally, an offline approach does not support interactive analysis wherein analysts immerse themselves in data and may dynamically select tags of interest during analysis, possibly using customized tagging functions of interest. 
%Tagging functions to extract such tags of interest   might not have been executed during offline processing. 
 
Our goal in this paper is to support interactive analysis on complex unstructured data that may not have been fully enriched either during the ingestion time or through an offline pre-processing step. We develop an approach entitled ``{\it Progressive Integrated Query Evaluation with Pay-as-you-go Enrichment}'' (PIQUE) that co-optimizes the process of enrichment with query evaluation.  A progressive approach refers to an online mechanism that enriches data in way that maximizes the rate at which the quality of the answer set of the query improves.
%
%By progressive approach, we mean an online mechanism that enriches data in such a way so as to maximize the rate at which the quality of the answer set for the query improves over time.
%improves the answer quality as quickly as possible so as to produce high-quality results if processing is stopped early. 
%A progressive approach can substantially reduce the query evaluation cost since the evaluation process can be prematurely terminated whenever a satisfactory level of quality is achieved.

Such a progressive approach is well suited for interactive analysis that needs to compute approximate results quickly (without having to wait for the entire data to be fully enriched) and can terminate the query whenever a satisfactory level of quality is achieved. 
Such a notion of progressiveness has been studied in the literature in various contexts such as in adaptive query processing through sampling~\cite{Karanasos:2014:DOQ:2588555.2610531,Markl:2004:RQP:1007568.1007642, Wu:2016:SQR:2882903.2882914}, in wavelet-based approximate query processing~\cite{Chakrabarti2001,Gilbert:2001:OAC:375551.375598}, and in data cleaning~\cite{Altowim:20F14:PAR:2732967.2732975,PayAsYouGoER,progressive-duplicate-detection, Raman:2001:PWI:645927.672045}. 

The main contribution of PIQUE is to prioritize/rank which tagging functions should be evaluated on which objects first in order to improve the quality of the answer set given a query as quickly as possible. To this end, PIQUE divides the query execution into several {\em epochs} and analyzes the evaluation progress at the beginning of each epoch to generate an execution plan for the current epoch. Such a plan consists of multiple {\em triples} 
that have the highest potential of improving the quality of the answer in that epoch, where a triple consists of an object, a query predicate, and a tagging function for evaluating the predicate on the object. 

PIQUE offers several benefits in the context of interactive analysis. It requires minimal data enrichment 
at the time of data ingestion (or as a pre-processing step prior to query execution); it only needs to execute a cheap tagging function that can be used to guide the joint enrichment and query execution. Furthermore, since it merges query execution and data enrichment into a single step, the data is available for analysis immediately after ingestion. Also, it allows analysts to specify and use sophisticated enrichment functions of their choice (that might not have been evaluated at ingestion time) for the purpose of tagging. 

%It does not require complex functions to be executed on the objects during the ingestion time reducing the ingestion time. Furthermore, it does not rely on any batched execution of these functions as a separate pre-processing step resulting in higher availability of these objects.   

PIQUE is motivated by several real-life scenarios; two of which are listed below:

\vspace{0.1cm}
\noindent
{\bf Scenario 1:} Consider a smart building deployment\footnote{This query is based on our experience in creating a smart IoT test bed at Donald Bren Hall of UCI~\cite{tippers}} wherein a diverse set of sensors are deployed to track the movement of people inside the buildings. Analysis of Wi-Fi signal might provide a cheap (but relatively coarse) localization of the people whereas face detection/recognition over images captured by hundreds of cameras installed within the building may offer an accurate, albeit more expensive, alternative. Exhaustive analysis of continuously captured video is likely computationally infeasible and/or wasteful. Instead, PIQUE answers queries based on subjects' location progressively by performing expensive video analysis on a selective portion of the data that helps in answering the query. 

\vspace{0.1cm}
\noindent
{\bf Scenario 2:} Consider a tweet monitoring system~\cite{tweet_topic_follow_up_demo} that tracks events in real-time over social media. Different tagging functions may be used to determine the tweet topics, the location where the tweet was posted from, references to locations in the text (if any), the sentiment/tone of the tweets, etc. While cheap variants of tagging functions for such enrichment tasks may exist,  tagging functions achieving a high-quality labelling  may incur significant computational costs. A user may be interested in analyzing social media posts (e.g., determining the geographical regions where the sentiment of tweets for a specific topic/event is mostly positive). Such analysis will require executing several tagging functions -- topic determination, location determination, and sentiment detection. PIQUE selectively chooses a set of tweets for each of these enrichment tasks with the goal of progressively answering the query. 

%Explain hw PIQUE helps here.... or give a different example where it helps.


%For example, real-time surveillance applications may require almost near real-time analysis to catch a suspect who is at the verge of escaping a crime scene. Although the required enrichment can be done accurately with sophisticated deep learning models to extract the frames of the suspect, fast processing can tremendously improve the chance of the suspect being detained. Stock-market traders might benefit from a quick analysis on the stock trends of the day rather than enriching the data to its entirety. News agencies can benefit from a quick analysis of the social media posts such as tweets, blogs to provide valuable insights during live events.   

%\vspace{0.1cm}
%\noindent
%\textbf{Scenario 1: } 
%Imagine an analyst interested in retrieving specific images of a particular event from social media (e.g., images containing people matching the description of a suspect during an incident). This will require us to analyze the images using various image processing techniques such as object detection \cite{object_detection}, person detection \cite{person_detection} and face detection \cite{face_detection_2}.

% Imagine a surveillance application 
%
\begin{comment}
For example, real-time surveillance applications may require almost near real-time analysis to catch a suspect who is at the verge of escaping a crime scene. Although the required enrichment can be done accurately with sophisticated deep learning models to extract the frames of the suspect, fast processing can tremendously improve the chance of the suspect being detained. Stock-market traders might benefit from a quick analysis on the stock trends of the day rather than enriching the data to its entirety.   

For example, anti-terrorism applications may require almost real-time analysis (where
streaming data are processed in small batches using
operations like ER) to capture a suspect who is on the brink
of escaping. Although the analysis may not be as complete
as when the full data are available, the fast processing can
increase the chance of the suspect being captured. As
another example, a news feed entity matching algorithm
may have very limited time for resolving company names
and individuals in a stock market trading scenario where
financial data are generated with high frequency.
\end{comment}

%The main idea of our progressive approach is to prioritize/rank which tags should be evaluated on which objects first in order to improve the quality of the answer set as quickly as possible.



In summary, our contributions in this paper are as follows:

%\noindent In summary, our primary contribution in this paper is a progressive approach to data enrichment and query processing entitled PIQUE. PIQUE makes several contributions:  
%contributions in this paper are as follows:

\begin{itemize}[leftmargin=*]
%\vspace{-0.2cm}
%\itemsep-0.2em 

%\item We develop a mechanism to jointly optimize data enrichment and query processing in order to progressive compute answers.

\item We propose a progressive approach to data enrichment and query evaluation entitled PIQUE that quantizes the execution time into epochs that are adaptively enriched. 
   
\item We present an algorithm for the problem of generating an execution plan that has the highest potential of improving the quality of the answer set in the corresponding epoch.
       
\item We develop an efficient probabilistic strategy for estimating the benefit of applying various tagging functions on different objects.


%\item We present an efficient strategy to estimate the benefits of the possible triples (i.e., object-predicate-function triple) \yat{ rest should be removed} based on different properties (i.e., output of previous functions, cost and quality of remaining functions).    
    
\item We experimentally evaluated PIQUE in different domains (i.e., images and tweets) using real datasets and tagging functions and demonstrate the efficiency of our solution.

%%%%%%%%%%%%%%

\end{itemize}



\begin{comment}

The past two decades have witnessed a rapid growth of data in the modern information systems in the form of text, images, video, and sensor readings. %The past two decades have witnessed a rapid growth of data on the Web.
Today, the Web hosts several billion web pages\footnote{According to reports such as~\cite{OnlineLiveStat}, users search roughly three Billion web pages per day using Google’s search engine.}, many of which contain rich multimodal content -- text, images, video, and tabular data. In addition, microblog sites such as Twitter generate data in the order of approximately 350K tweets/minute, Instagram users upload~200K images/min, and YouTube receives~300~hours of uploaded video every minute~\cite{OnlineLiveStat}. This explosion of data has spurred significant advances in machine learning, natural language processing, image processing, etc., to enrich data with semantic tags that can enable powerful query processing techniques that go well beyond the existing query processing techniques present in today’s information systems. Our goal in this paper is to perform query processing on such datasets using such tagging functions. The following examples illustrate the benefits of semantic tagging of objects:

%Queries over such data arise in several domains such as social media analysis, multimedia data analysis, and Internet-of-Things applications. However, such data is often too low-level for the end applications due to the existing semantic gap and hence need to be further enriched/tagged before they can be queried. 


\vspace{0.1cm}
\noindent
\textbf{Scenario 1: } 
Imagine an analyst interested in retrieving specific images of a particular event from social media (e.g., images containing people matching the description of a suspect during an incident). This will require us to analyze the images using various image processing techniques such as object detection \cite{object_detection}, person detection \cite{person_detection} and face detection \cite{face_detection_2}.


\vspace{0.1cm}
\noindent
\textbf{Scenario 2: } 
Let us consider an exploratory analysis tool built around user generated data such as reviews and tweets. An analyst might  wish to study the reaction of societal events through such content (e.g., acceptance of a new product by the public). This will require analyzing the sentiment of user content using techniques such as \cite{sentiment_analysis_classifiers}. 




\vspace{0.1cm}
\noindent
\textbf{Scenario 3:} 
Imagine a user is searching for websites about a specific topic (e.g., a person or a product). Default search method in modern search engines is key-word based search. Such techniques will fail in the context of ambiguity (e.g., ``apple'' could be related to the fruit or the company). Different entity disambiguation-based techniques have been proposed in the literature~\cite{entity_search_1,person_search_1,resource_selection_1} to address this issue. Tagging based on these techniques can help the process of query evaluation.







Since tagging functions (e.g., sentiment analysis, image processing, entity disambiguation, or a combination of all) are often uncertain in nature and the quality of the tags often increase using more expensive techniques, it is difficult to decide the right degree of enrichment. To support scenarios like the above and others, the different enrichment functions will have to be performed on all the objects and/or for all the possible entities. Such an approach, if at all possible given the computational resources required, is sub-optimal from several perspectives. First, data cannot be retrieved based on tags until it is enriched. Second, the enrichment process will be wasteful if its result is not used by any queries. Third, enrichment is a continuous process and the right degree of enrichment mainly depends on the query.




This paper explores a radically different approach that, depending on the query, enriches a subset of the objects online at the query processing time, to improve the quality of the results in a pay-as-you-go fashion. Often the enrichment process that combines the results of multiple tagging functions can reduce the uncertainty of tags~\cite{Domingos96usingpartitioning,Opitz99popularensemble,Quinlan:1996:BBC:1892875.1892983} albeit at higher computational cost. Our combined enrichment and query processing technique determines which object(s) to tag using which tagging functions in order to optimize the quality of answer progressively. 


By progressive approach, we mean an online approach that improves the answer quality as quickly as possible so as to produce high-quality results if processing is stopped early. A progressive approach can substantially reduce the query evaluation cost since the evaluation process can be prematurely terminated whenever a satisfactory level of quality is achieved. Such a notion of progressive evaluation has been studied in the literature in various contexts such as in adaptive query processing through sampling~\cite{Karanasos:2014:DOQ:2588555.2610531,Markl:2004:RQP:1007568.1007642, Wu:2016:SQR:2882903.2882914}, in wavelet-based approximate query processing~\cite{Chakrabarti2001,Gilbert:2001:OAC:375551.375598}, and in data cleaning~\cite{Altowim:20F14:PAR:2732967.2732975,PayAsYouGoER,progressive-duplicate-detection, Raman:2001:PWI:645927.672045}. 
 



The main idea of our progressive approach is to prioritize/rank which tags should be evaluated on which objects first in order to improve the quality of the answer set as quickly as possible. To this end, our approach divides the query execution time into several $epochs$ and analyzes the evaluation progress at the beginning of each epoch to generate an execution plan for the current epoch. An evaluation plan consists of multiple triples %(\yat{is it triple or triple???})) 
that have the highest potential of improving the quality of the answer in that epoch, where a triple consists of an object, a query predicate, and a tagging function for evaluating the predicate on the object. 



\noindent In summary, our contributions in this paper are as follows:
\begin{itemize}[leftmargin=*]
\itemsep-0.2em 
\item We propose a progressive approach to data enrichment and query evaluation.
   
\item We present an algorithm for the problem of generating an execution plan that has the highest potential of improving the quality of the answer set in the corresponding epoch.
       
\item We present an efficient strategy that estimates the benefits of the possible triples (i.e., object-predicate-function triple) based on different properties (i.e., output of previous functions, cost and quality of remaining functions).    
    
\item We experimentally evaluated our approach in different domains (i.e., images and tweets) using real datasets and tagging functions and demonstrate the efficiency of our proposed solution.
\end{itemize}
\end{comment}

%%%% SIGMOD Introduction %%%%%%%

%\vspace{1cm}

\begin{comment}
\section{Introduction (SIGMOD)}
\label{sect:introduction}

Modern information systems often collect raw data in the form of text, images, video, and sensor readings. Queries over such data arise in several domains such as social media analysis, multimedia data analysis, and Internet-of-Things applications. However, such data is often too low-level for the end applications due to the existing semantic gap and hence need to be further enriched/tagged before they can be queried. 

Given the large amount of data, such tags are generated using automated functions (e.g., pre-trained classifiers) and/or data extraction or analysis mechanisms (e.g., sentiment detection) and hence are often uncertain.


The amount of uncertainty present in the generated tags depends on the cost and quality of these tagging functions. A more expensive tagging function usually produces better quality tags (i.e., tags with less uncertainty). For instance, executing a tagging function that combines the results of multiple tagging functions, although computationally expensive, has been shown to reduce the uncertainty of tags~\cite{Domingos96usingpartitioning,Opitz99popularensemble,Quinlan:1996:BBC:1892875.1892983}. 



Our goal in this paper is to perform query processing on such datasets using such tagging functions. Query processing would be simple if the underlying dataset could be pre-tagged prior to the arrival of queries. However, there are several reasons why such pre-tagging is not possible. First and foremost, pre-tagging a dataset requires that we exactly know a priori all the analysis tasks that we want to implement over the dataset in the future. Let us consider an example of a dataset of surveillance camera images and a query for catching a perpetrator of a theft. The fact that one is interested in a person with a purple shirt with a backpack might be a result of a memory of a person who saw someone suspicious that instigated the query\footnote{{This example is inspired by a real occurrence in the authors' Department building wherein the research infrastructure of cameras was used to create an image profile of a perpetrator who stole several computers, iPads, and phones from several offices.}}. It is virtually impossible to know that such an analysis query would be of interest beforehand. Second, even if we have created the tags for each object, we might not have used the most accurate tagging function for generating those tags which will result in low quality results. 


Motivated by the above scenarios, we propose a progressive approach to data enrichment and query evaluation. Figure~\ref{fig:ProgressiveEvaluation} illustrates the concept of progressive evaluation and how it differs from traditional and incremental evaluation approaches. In the traditional approach, all the required tagging functions are executed on all the objects first before answering any query. In this scenario, the quality of the result will stay low for a long time (i.e., until all the tags have been generated using all the tagging functions and for all the objects) and then reaches a very high value. Answering a query using this approach will take a large amount of time especially if the dataset is large and/or the number of tags and the number of functions for evaluating those tags are large. In the incremental evaluation, the algorithm is configured to constantly improve the quality of the answer by improving the quality of the tags of objects. 
%trim={1.1cm 0.8cm 1cm 1.32cm},clip,
%%%%%%%%%% Progressive Approach Figure %%%%%%
\begin{figure}[t]
	\centering
     \includegraphics[trim={1.1cm 0.5cm 1cm 0.1cm},clip, width=0.32\textwidth,height=0.22\textwidth]{ProgressiveApproach/ProgressiveApproach_plot2.eps}
    %\includegraphics[width=2cm]{ProgressiveApproach/ProgressiveApproach_plot2.eps}
\vspace{-0.2cm}
\caption{Different evaluation approaches.}

\label{fig:ProgressiveEvaluation}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Both of these approaches are not suitable for applications that require low latency response (and thus cannot tolerate delays caused by generating accurate tags for each object), and/or interactive applications that need to show preliminary analysis results based on moderately tagged objects and progressively refine their results by executing more tagging functions to improve the tagging accuracy. On the other hand, a progressive approach aims to improve the quality of the tags in such a way so that the rate at which the quality of the answer set improves is maximized. Such an approach can substantially reduce the query evaluation cost since the evaluation process can be prematurely terminated whenever a satisfactory level of quality is achieved. Progressive evaluation has been studied in the literature in various contexts such as in adaptive query processing through sampling~\cite{Karanasos:2014:DOQ:2588555.2610531,Markl:2004:RQP:1007568.1007642, Wu:2016:SQR:2882903.2882914}, in wavelet-based approximate query processing~\cite{Chakrabarti2001,Gilbert:2001:OAC:375551.375598}, and in data cleaning~\cite{Altowim:20F14:PAR:2732967.2732975,PayAsYouGoER,progressive-duplicate-detection, Raman:2001:PWI:645927.672045}. 

The main idea of our progressive approach is to prioritize/rank which tags should be evaluated on which objects first in order to improve the quality of the answer set as quickly as possible. To this end, our approach divides the query execution time into several $epochs$ and analyzes the evaluation progress at the beginning of each epoch to generate an execution plan for the current epoch. An evaluation plan consists of multiple triples %(\yat{is it triple or triple???})) 
that have the highest potential of improving the quality of the answer in that epoch, where a triple consists of an object, a query predicate, and a tagging function for evaluating the predicate on the object. 


\noindent In summary, our contributions in this paper are as follows:
\begin{itemize}[leftmargin=*]
\itemsep-0.2em 
\item We propose a progressive approach to data enrichment and query evaluation.
   
\item We present an algorithm for the problem of generating an execution plan that has the highest potential of improving the quality of the answer set in the corresponding epoch.
       
\item We present an efficient strategy that estimates the benefits of the possible triples (i.e., object-predicate-function triple) based on different properties (i.e., output of previous functions, cost and quality of remaining functions).    
    
\item We experimentally evaluated our approach in different domains (i.e., images and tweets) using real datasets and tagging functions and demonstrate the efficiency of our proposed solution.
\end{itemize}
%%2
\end{comment}

\begin{comment}

%%% Previous introduction. 
%We consider the problem of execution of selection queries containing predicates defined over tags that objects can contain, in a large collection of objects. 

We consider the problem of execution of queries containing predicates defined over tags which objects can contain in a large collection of objects. Queries over tagged uncertain data arise in several domains such as twitter analysis, multimedia data analysis, Internet-Of-Things. Data generated in these domains (e.g., tweets, photos, texts, sensor data) is usually too low-level for end applications due to the existing semantic gap. Hence, such data needs to be analyzed and tagged in order to be useful. Given the large amount of data, such tags are often results of automated analysis, e.g., pre-trained classifiers and/or mechanisms for data extraction or analysis such as sentiment detection, and as such contain some uncertainty. 

Indeed, the amount of uncertainty present in the generated tags depends on the cost and quality of these tagging mechanisms: usually a more expensive tagging function produces better quality tags (i.e., tags with less uncertainty). For instance, executing more than one tagging function and combining their results, even when computationally costly, has been shown to reduce the uncertainty of tags~\cite{Domingos96usingpartitioning,Opitz99popularensemble,Quinlan:1996:BBC:1892875.1892983}. As an example, Table \ref{table:example_function} shows the trade-off between quality and cost of different tagging functions for extracting gender from images: Decision Tree classifier, Gaussian Naive-Bayes classifier and Support Vector Machine classifier on two real datasets that we have used in our experiments.
%Furthermore there exists a trade-off between the cost and quality of these tagging functions and also in the combinations of these tagging functions. Combining cheaper tagging functions will produce low quality answer where as combining expensive functions will produce high quality answer. 
%\hl{As an example, in our experimental evaluation we show the trade off between quality and cost of different classifier to detect X in images (see Figure~X). Notice that the figure also shows how the combination of the classifiers obtains the best results but increase the cost significantly.}

\begin{table}[!htb]
\small
\centering
\begin{center}
 \begin{tabular}{|c c c c|} 
 \hline
  Dataset &Function & Quality(AUC) & Cost (Sec)\\ 
 \hline
 MUCT & DT & 0.61 & 0.023 \\ 
 \hline
 MUCT & GNB & 0.67 & 0.114 \\
 \hline
 MUCT & SVM & 0.71 & 0.949 \\
 \hline
 Multi-PIE & DT & 0.53 & 0.018 \\  
 \hline
  Multi-PIE & GNB & 0.84 & 0.096 \\  
 \hline
  Multi-PIE & SVM & 0.89 & 0.886 \\  
 \hline
\end{tabular}
\caption{Cost and quality of different tagging functions for tag type {\tt Gender} on two real datasets.}
\label{table:example_function}
\end{center}
\end{table}


 

%paid during execution of the tagging functions. If the cost paid is more by it will reduce the uncertainty of the generated tags more.
%In addition to generating tags using a single tagging function, the querier might want to execute more than one tagging functions to increase the overall quality of the tags and the answer. The combination of output of such functions has been known to reduce the uncertainty in different scenarios \cite{Domingos96usingpartitioning}\cite{Opitz99popularensemble}\cite{Quinlan:1996:BBC:1892875.1892983}. Furthermore there exists a trade-off between the cost and quality of these tagging functions and also in the combinations of these tagging functions. Combining cheaper tagging functions will produce low quality answer where as combining expensive functions will produce high quality answer.  
Our goal in this paper is to perform query processing on such datasets and with such tagging functions. Query processing would be simple if the underlying data could be pre-tagged prior to the arrival of queries. But there are several reasons why such pre-tagging is not possible. First and foremost, pre-tagging a corpus requires that we exactly know all the functions that we want to implement over it. While one may have an idea of some of the analysis tasks of interest, it is virtually impossible to know a priori all the future use of data. Let us consider an example of a dataset of surveillance camera images and a query for catching a perpetrator of a theft. The fact that one is interested in a person with a purple shirt with a backpack might be a result of a memory of a person who saw someone suspicious that instigated the query\footnote{This example is inspired by a real occurrence in the authors' Computer Science Department building wherein the research infrastructure of cameras was used to create an image profile of a perpetrator who stole several computers, iPads, and phones from several offices.}. There is no way to know that such an analysis query would be of interest beforehand. Secondly, even if we have created the tags for each object, we might not have used the most accurate tagging function for generating those tags which will result low quality results. 



%\hl{In the following paragraph we have to motivate why the approach should be progressive. I added a sentence explaining why a traditional approach is not feasible, but why wouldn't an iterative approach suffice?}
%Specifically our goal is to develop a progressive approach where we tag the right set of objects using the right set of tagging functions.
Motivated by the above scenarios, we propose a progressive approach for evaluating these queries.
Figure~\ref{fig:ProgressiveEvaluation} depicts the concept of progressive evaluation and how it differs from traditional and incremental evaluations. In a traditional evaluation, all the required tagging functions are executed on the objects first for generating highest quality tags before answering any query. In this scenario, the quality of the result will stay low for a long time (i.e., until all the tags have been generated using all the tagging functions and for all the objects) and then reaches to a very high value. This would not be useful because if the dataset is large and/or the number of functions for evaluating tags and number of tags are large, then it will take a large amount of time to be able to answer a query. 
In an ``incremental'' algorithm, the algorithm is configured to constantly improve the quality of the result by improving the quality of the tags of objects. However, both of these approaches are not suitable for applications that require low latency response (and thus cannot tolerate delays caused by generating most accurate tags for each objects), and/or interactive applications that need to show preliminary analysis results based on the moderately tagged objects and progressively refine their results by executing more tagging functions and generating more accurate tags. On the other hand, a progressive approach aims to improve the quality of the tags in such a way so that the rate at which the quality of the answer set improves is maximized.  Progressive evaluation has been studied in the literature in various contexts such as progressive adaptive query processing through sampling~\cite{Karanasos:2014:DOQ:2588555.2610531,Markl:2004:RQP:1007568.1007642, Wu:2016:SQR:2882903.2882914}, wavelet based approximate query processing~\cite{Chakrabarti2001,Gilbert:2001:OAC:375551.375598}, and in progressive data cleaning~\cite{Altowim:20F14:PAR:2732967.2732975,PayAsYouGoER,progressive-duplicate-detection, Raman:2001:PWI:645927.672045}. 

%in a scenario where the dataset, as well as the number of tags to extract per object and tagging functions per tag, are large. 
%The idea of progressive approaches have been used in the database literature before in the context of progressive data cleaning ~\cite{Altowim:20F14:PAR:2732967.2732975,PayAsYouGoER,progressive-duplicate-detection}.adaptive query processing \cite{DBS-001},


In our progressive approach the main goal is to prioritize/rank which part of the dataset should be chosen first for improving the quality of the tags, so that the quality of the answer set improves as early as possible during the query execution time. With a progressive evaluation, the total cost of generating tags can be substantially reduced, as the query execution can be terminated at any time based on the achieved level of quality. %In the next paragraph we compare progressive approach with traditional approaches and incremental approaches.




%%%%%%%%%% Progressive Approach Figure %%%%%%
\begin{figure}[htb]
	\centering
    %0.25\textwidth[width=0.5\hsize]
	\includegraphics[width=0.36\textwidth]{ProgressiveApproach/ProgressiveApproach_plot2.eps}
    %\includegraphics[decodearray={0.2 0.5}]{ProgressiveApproach/ProgressiveApproach_quality.eps}
\caption{Comparison of query evaluation approaches: Traditional vs Incremental vs Progressive.}
\label{fig:ProgressiveEvaluation}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We formalize progressiveness by dividing the query execution time into several $epochs$ and our goal translates into processing the best set of (object, tagging function) pairs in each epoch so that the rate at which quality of the answer set improves is maximized. Also each epoch has different importance: the epochs in the beginning of the query execution have higher importance as compared to the ones in the later part of the execution. To this end, we assign a weight value to each epoch starting with the highest weight assigned to the first epoch. Using these weight values, we have modeled the goal of our progressive evaluation as an optimization problem which maximizes a function of the quality of the answer at the end of different $epochs$. The weight function is monotonically decreasing starting with the highest value in the first epoch. 

%\hl{We lack a paragraph here that summarizes our approach. The same paragraph should explain the limitations: Although the main focus of our approach is on selections because... and the approach considers that the dataset is stored in main memory before processing, we explain how the technique could be generalized to address these issues. }

 Our approach divides an epoch into two phases: plan generation phase and plan execution phase. A plan consists of multiple triples where each triple consists of an object, a predicate and a tagging function for evaluating the predicate. In each epoch, our approach identifies a set of triples which have the highest potential of improving the quality of the answer in that epoch. 
 
% In developing our approach we have considered several assumptions about the queries and the data. We have considered the queries to be selection queries as they are the most commonly used queries. Regarding size of the dataset, we have assumed that the set of objects in the dataset for which tagging has to be performed, can fit in memory. Furthermore, we have 
%assumed that for each of these objects, one tagging function (cheapest) of the available tag types, is already executed at the arrival time of the object as a preprocessing step. We explain how our approach can be generalized to address these issues in section \ref{sect:extensions}. In join queries, we have assumed that the conditions of join predicate, contain attributes other than the tagged attributes.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Updated assumptions paragraph. (Based on Sharad's feedback)

In developing our approach we have considered several assumptions about the data and the queries. We have considered the queries to be general \emph{Select-Project-Join} type of queries with an assumption on join predicates. In join predicates, we have assumed that the join condition does not contain any tagged attributes as they are approximate and contain uncertainty. We assume that none of the objects are preprocessed with any tagging functions before the arrival of a query (except for some basic preprocessing). Regarding the size of the dataset, we consider that the set of objects in the dataset for which tagging has to be performed, can fit in memory. We explain how our approach can be generalized to remove these assumptions in Section \ref{sect:extensions}.
 
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

%Furthermore, there are plenty of situations in which queries have to be answered in near real-time. For instance, a journalist covering a live presidential debate might want to analyze in real-time the sentiment of the tweets posted in last one hour from a certain state about a certain topic before the candidates move into the next topic in the debate. Such query has to be answered near real time so that  it can be used in the live coverage of the show. As tweets are not tagged with sentiment or the particular topic of the discussion in the debate, the journalist has to execute some sentiment analysis codes and topic detection codes for determining these predicates. This implies that answering such queries in near real time where some of the tags are derived in query time becomes challenging.



%Based on the above scenarios, where pre-tagging a corpus is not a feasible option and near-real time query answering is a mandatory criteria, we propose a progressive approach for evaluating these queries. Such an approach serves the purposes of both low latency query response time and eliminates the need of pre-tagging an entire corpus. The main idea of progressive approach is to prioritize/rank which part of the dataset should be chosen first for improving the quality of the tags, so that the quality of the answer set improves as early as possible during the query execution time.     



%Figure \ref{fig:ProgressiveEvaluation} depicts the concept of progressive evaluation and how it differs from traditional and incremental evaluations. In a traditional evaluation, all the required tagging functions are executed on the objects first for generating highest quality tags and then query results are returned. In this scenario, the quality of the result stays low for a long time and then reaches to a very high value. In an  ``incremental'' algorithm, the algorithm is configured to constantly improve the quality of the result by improving the quality of the tags of objects. On the other hand, progressive approach aims to improve the quality of the tags in such a way so that the rate at which the quality of the answer set improves is maximized. The idea of progressive approaches have been used in the database literature before in the context of progressive entity resolution ~\cite{Altowim:20F14:PAR:2732967.2732975,PayAsYouGoER,progressive-duplicate-detection}. In the next paragraph, we explain the goals of our progressive approach.


%Such progressive approaches have been used in the context of progressive entity resolution before ~\cite{Altowim:20F14:PAR:2732967.2732975,PayAsYouGoER,progressive-duplicate-detection}.

%~\cite{progressive-duplicate-detection,Altowim:20F14:PAR:2732967.2732975}


%In our progressive approach, a certain time interval is setup by a domain expert (denoted as $interval$), which implies that the user is expecting an answer after every $interval$ unit of time. The goal of a progressive algorithm translates into generating an answer at every $interval$, so that the rate of quality improvement of the answer, is maximized. We have modeled this goal as an optimization problem which maximizes a quality function $Qty(A)$, where $Qty(A)$ is a function of the quality of the answer at the end of different $intervals$. In the function $Qty(A)$, we assign a certain weight value to each $interval$ where the weight function is a monotonically decreasing function starting from the highest value at the first interval after the beginning of query execution.



\noindent In summary, our contributions in this paper are as follows:

\begin{itemize}[leftmargin=*]
\itemsep-0.2em 
	
    
    \item We propose an approach to progressive processing of queries with predicates containing tags of different tag types, over tagged datasets.
    
    \item We present an algorithm to generate execution plans including triples object-predicate-function (i.e., which predicate of which object has to be evaluated with which tagging function) which have the highest potential to improve the quality of the answer set in each epoch.
   
    %\item We present an algorithm to choose a set of objects in each epoch as candidate objects which have higher probability of increasing the quality of the answer set in that epoch.
    
    \item We present an efficient strategy to estimate the benefits of the possible triples (i.e., object-predicate-function triple) to compare between them, by leveraging different properties of such triples (i.e., output of previous functions, cost and quality of remaining functions etc.).
    
    
    
    \item We experimentally evaluated our approach using real datasets and tagging functions in different domains (i.e., tweets and images) and demonstrate the efficiency of our approach.
    %\item We propose an approach to progressive processing of queries with predicates that involve tags over untagged datasets.
    
    % \item We present an algorithm to generate execution plans including triples object-predicate-function (i.e., which predicate of which object has to be evaluated with which tagging function) that should be run in order to maximize the quality of the answer of the query.
    
    %\item We present an algorithm to generate execution plans in each epoch that consists of a set of object-predicate-function triples(i.e., which object should be evaluated and with which  tagging function of a predicate) that have the highest potential to improve the quality of the answer set in that epoch.
    
    %\item We present a mechanism to estimate the benefit of a possible triple object-predicate-function using information extracted about the cost and quality of the different functions.%\hl{Remember to add some sneak peek of the results.}

\end{itemize}

The rest of the paper is organized as follows. 
In Section~\ref{sect:problemDefinition}, we define the notation and problem.
In Section~\ref{sect:overview}, we present an overview of the approach.
In Section~\ref{sect:plan generation}, we detail our mechanism to generate and execute plans which has the highest capability of improving the quality of the answer set in each epoch.
In Section~\ref{sect:extensions}, we introduce some extensions to our approach.
In Section~\ref{sect:experiments}, we show the experimental evaluation performed to validate our approach.
Finally, Section~\ref{sect:relatedWork} surveys related works and Section~\ref{sect:conclusions} presents conclusions and future work.
\end{comment}  
%sigmod



\begin{comment}

%%% Previous introduction. 
%We consider the problem of execution of selection queries containing predicates defined over tags that objects can contain, in a large collection of objects. 

We consider the problem of execution of queries containing predicates defined over tags which objects can contain in a large collection of objects. Queries over tagged uncertain data arise in several domains such as twitter analysis, multimedia data analysis, Internet-Of-Things. Data generated in these domains (e.g., tweets, photos, texts, sensor data) is usually too low-level for end applications due to the existing semantic gap. Hence, such data needs to be analyzed and tagged in order to be useful. Given the large amount of data, such tags are often results of automated analysis, e.g., pre-trained classifiers and/or mechanisms for data extraction or analysis such as sentiment detection, and as such contain some uncertainty. 

Indeed, the amount of uncertainty present in the generated tags depends on the cost and quality of these tagging mechanisms: usually a more expensive tagging function produces better quality tags (i.e., tags with less uncertainty). For instance, executing more than one tagging function and combining their results, even when computationally costly, has been shown to reduce the uncertainty of tags~\cite{Domingos96usingpartitioning,Opitz99popularensemble,Quinlan:1996:BBC:1892875.1892983}. As an example, Table \ref{table:example_function} shows the trade-off between quality and cost of different tagging functions for extracting gender from images: Decision Tree classifier, Gaussian Naive-Bayes classifier and Support Vector Machine classifier on two real datasets that we have used in our experiments.
%Furthermore there exists a trade-off between the cost and quality of these tagging functions and also in the combinations of these tagging functions. Combining cheaper tagging functions will produce low quality answer where as combining expensive functions will produce high quality answer. 
%\hl{As an example, in our experimental evaluation we show the trade off between quality and cost of different classifier to detect X in images (see Figure~X). Notice that the figure also shows how the combination of the classifiers obtains the best results but increase the cost significantly.}

\begin{table}[!htb]
\small
\centering
\begin{center}
 \begin{tabular}{|c c c c|} 
 \hline
  Dataset &Function & Quality(AUC) & Cost (Sec)\\ 
 \hline
 MUCT & DT & 0.61 & 0.023 \\ 
 \hline
 MUCT & GNB & 0.67 & 0.114 \\
 \hline
 MUCT & SVM & 0.71 & 0.949 \\
 \hline
 Multi-PIE & DT & 0.53 & 0.018 \\  
 \hline
  Multi-PIE & GNB & 0.84 & 0.096 \\  
 \hline
  Multi-PIE & SVM & 0.89 & 0.886 \\  
 \hline
\end{tabular}
\caption{Cost and quality of different tagging functions for tag type {\tt Gender} on two real datasets.}
\label{table:example_function}
\end{center}
\end{table}


 

%paid during execution of the tagging functions. If the cost paid is more by it will reduce the uncertainty of the generated tags more.
%In addition to generating tags using a single tagging function, the querier might want to execute more than one tagging functions to increase the overall quality of the tags and the answer. The combination of output of such functions has been known to reduce the uncertainty in different scenarios \cite{Domingos96usingpartitioning}\cite{Opitz99popularensemble}\cite{Quinlan:1996:BBC:1892875.1892983}. Furthermore there exists a trade-off between the cost and quality of these tagging functions and also in the combinations of these tagging functions. Combining cheaper tagging functions will produce low quality answer where as combining expensive functions will produce high quality answer.  
Our goal in this paper is to perform query processing on such datasets and with such tagging functions. Query processing would be simple if the underlying data could be pre-tagged prior to the arrival of queries. But there are several reasons why such pre-tagging is not possible. First and foremost, pre-tagging a corpus requires that we exactly know all the functions that we want to implement over it. While one may have an idea of some of the analysis tasks of interest, it is virtually impossible to know a priori all the future use of data. Let us consider an example of a dataset of surveillance camera images and a query for catching a perpetrator of a theft. The fact that one is interested in a person with a purple shirt with a backpack might be a result of a memory of a person who saw someone suspicious that instigated the query\footnote{This example is inspired by a real occurrence in the authors' Computer Science Department building wherein the research infrastructure of cameras was used to create an image profile of a perpetrator who stole several computers, iPads, and phones from several offices.}. There is no way to know that such an analysis query would be of interest beforehand. Secondly, even if we have created the tags for each object, we might not have used the most accurate tagging function for generating those tags which will result low quality results. 



%\hl{In the following paragraph we have to motivate why the approach should be progressive. I added a sentence explaining why a traditional approach is not feasible, but why wouldn't an iterative approach suffice?}
%Specifically our goal is to develop a progressive approach where we tag the right set of objects using the right set of tagging functions.
Motivated by the above scenarios, we propose a progressive approach for evaluating these queries.
Figure~\ref{fig:ProgressiveEvaluation} depicts the concept of progressive evaluation and how it differs from traditional and incremental evaluations. In a traditional evaluation, all the required tagging functions are executed on the objects first for generating highest quality tags before answering any query. In this scenario, the quality of the result will stay low for a long time (i.e., until all the tags have been generated using all the tagging functions and for all the objects) and then reaches to a very high value. This would not be useful because if the dataset is large and/or the number of functions for evaluating tags and number of tags are large, then it will take a large amount of time to be able to answer a query. 
In an ``incremental'' algorithm, the algorithm is configured to constantly improve the quality of the result by improving the quality of the tags of objects. However, both of these approaches are not suitable for applications that require low latency response (and thus cannot tolerate delays caused by generating most accurate tags for each objects), and/or interactive applications that need to show preliminary analysis results based on the moderately tagged objects and progressively refine their results by executing more tagging functions and generating more accurate tags. On the other hand, a progressive approach aims to improve the quality of the tags in such a way so that the rate at which the quality of the answer set improves is maximized.  Progressive evaluation has been studied in the literature in various contexts such as progressive adaptive query processing through sampling~\cite{Karanasos:2014:DOQ:2588555.2610531,Markl:2004:RQP:1007568.1007642, Wu:2016:SQR:2882903.2882914}, wavelet based approximate query processing~\cite{Chakrabarti2001,Gilbert:2001:OAC:375551.375598}, and in progressive data cleaning~\cite{Altowim:20F14:PAR:2732967.2732975,PayAsYouGoER,progressive-duplicate-detection, Raman:2001:PWI:645927.672045}. 

%in a scenario where the dataset, as well as the number of tags to extract per object and tagging functions per tag, are large. 
%The idea of progressive approaches have been used in the database literature before in the context of progressive data cleaning ~\cite{Altowim:20F14:PAR:2732967.2732975,PayAsYouGoER,progressive-duplicate-detection}.adaptive query processing \cite{DBS-001},


In our progressive approach the main goal is to prioritize/rank which part of the dataset should be chosen first for improving the quality of the tags, so that the quality of the answer set improves as early as possible during the query execution time. With a progressive evaluation, the total cost of generating tags can be substantially reduced, as the query execution can be terminated at any time based on the achieved level of quality. %In the next paragraph we compare progressive approach with traditional approaches and incremental approaches.




%%%%%%%%%% Progressive Approach Figure %%%%%%
\begin{figure}[htb]
	\centering
    %0.25\textwidth[width=0.5\hsize]
	\includegraphics[width=0.36\textwidth]{ProgressiveApproach/ProgressiveApproach_plot2.eps}
    %\includegraphics[decodearray={0.2 0.5}]{ProgressiveApproach/ProgressiveApproach_quality.eps}
\caption{Comparison of query evaluation approaches: Traditional vs Incremental vs Progressive.}
\label{fig:ProgressiveEvaluation}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We formalize progressiveness by dividing the query execution time into several $epochs$ and our goal translates into processing the best set of (object, tagging function) pairs in each epoch so that the rate at which quality of the answer set improves is maximized. Also each epoch has different importance: the epochs in the beginning of the query execution have higher importance as compared to the ones in the later part of the execution. To this end, we assign a weight value to each epoch starting with the highest weight assigned to the first epoch. Using these weight values, we have modeled the goal of our progressive evaluation as an optimization problem which maximizes a function of the quality of the answer at the end of different $epochs$. The weight function is monotonically decreasing starting with the highest value in the first epoch. 

%\hl{We lack a paragraph here that summarizes our approach. The same paragraph should explain the limitations: Although the main focus of our approach is on selections because... and the approach considers that the dataset is stored in main memory before processing, we explain how the technique could be generalized to address these issues. }

 Our approach divides an epoch into two phases: plan generation phase and plan execution phase. A plan consists of multiple triples where each triple consists of an object, a predicate and a tagging function for evaluating the predicate. In each epoch, our approach identifies a set of triples which have the highest potential of improving the quality of the answer in that epoch. 
 
% In developing our approach we have considered several assumptions about the queries and the data. We have considered the queries to be selection queries as they are the most commonly used queries. Regarding size of the dataset, we have assumed that the set of objects in the dataset for which tagging has to be performed, can fit in memory. Furthermore, we have 
%assumed that for each of these objects, one tagging function (cheapest) of the available tag types, is already executed at the arrival time of the object as a preprocessing step. We explain how our approach can be generalized to address these issues in section \ref{sect:extensions}. In join queries, we have assumed that the conditions of join predicate, contain attributes other than the tagged attributes.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Updated assumptions paragraph. (Based on Sharad's feedback)

In developing our approach we have considered several assumptions about the data and the queries. We have considered the queries to be general \emph{Select-Project-Join} type of queries with an assumption on join predicates. In join predicates, we have assumed that the join condition does not contain any tagged attributes as they are approximate and contain uncertainty. We assume that none of the objects are preprocessed with any tagging functions before the arrival of a query (except for some basic preprocessing). Regarding the size of the dataset, we consider that the set of objects in the dataset for which tagging has to be performed, can fit in memory. We explain how our approach can be generalized to remove these assumptions in Section \ref{sect:extensions}.
 
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

%Furthermore, there are plenty of situations in which queries have to be answered in near real-time. For instance, a journalist covering a live presidential debate might want to analyze in real-time the sentiment of the tweets posted in last one hour from a certain state about a certain topic before the candidates move into the next topic in the debate. Such query has to be answered near real time so that  it can be used in the live coverage of the show. As tweets are not tagged with sentiment or the particular topic of the discussion in the debate, the journalist has to execute some sentiment analysis codes and topic detection codes for determining these predicates. This implies that answering such queries in near real time where some of the tags are derived in query time becomes challenging.



%Based on the above scenarios, where pre-tagging a corpus is not a feasible option and near-real time query answering is a mandatory criteria, we propose a progressive approach for evaluating these queries. Such an approach serves the purposes of both low latency query response time and eliminates the need of pre-tagging an entire corpus. The main idea of progressive approach is to prioritize/rank which part of the dataset should be chosen first for improving the quality of the tags, so that the quality of the answer set improves as early as possible during the query execution time.     



%Figure \ref{fig:ProgressiveEvaluation} depicts the concept of progressive evaluation and how it differs from traditional and incremental evaluations. In a traditional evaluation, all the required tagging functions are executed on the objects first for generating highest quality tags and then query results are returned. In this scenario, the quality of the result stays low for a long time and then reaches to a very high value. In an  ``incremental'' algorithm, the algorithm is configured to constantly improve the quality of the result by improving the quality of the tags of objects. On the other hand, progressive approach aims to improve the quality of the tags in such a way so that the rate at which the quality of the answer set improves is maximized. The idea of progressive approaches have been used in the database literature before in the context of progressive entity resolution ~\cite{Altowim:20F14:PAR:2732967.2732975,PayAsYouGoER,progressive-duplicate-detection}. In the next paragraph, we explain the goals of our progressive approach.


%Such progressive approaches have been used in the context of progressive entity resolution before ~\cite{Altowim:20F14:PAR:2732967.2732975,PayAsYouGoER,progressive-duplicate-detection}.

%~\cite{progressive-duplicate-detection,Altowim:20F14:PAR:2732967.2732975}


%In our progressive approach, a certain time interval is setup by a domain expert (denoted as $interval$), which implies that the user is expecting an answer after every $interval$ unit of time. The goal of a progressive algorithm translates into generating an answer at every $interval$, so that the rate of quality improvement of the answer, is maximized. We have modeled this goal as an optimization problem which maximizes a quality function $Qty(A)$, where $Qty(A)$ is a function of the quality of the answer at the end of different $intervals$. In the function $Qty(A)$, we assign a certain weight value to each $interval$ where the weight function is a monotonically decreasing function starting from the highest value at the first interval after the beginning of query execution.



\noindent In summary, our contributions in this paper are as follows:

\begin{itemize}[leftmargin=*]
\itemsep-0.2em 
	
    
    \item We propose an approach to progressive processing of queries with predicates containing tags of different tag types, over tagged datasets.
    
    \item We present an algorithm to generate execution plans including triples object-predicate-function (i.e., which predicate of which object has to be evaluated with which tagging function) which have the highest potential to improve the quality of the answer set in each epoch.
   
    %\item We present an algorithm to choose a set of objects in each epoch as candidate objects which have higher probability of increasing the quality of the answer set in that epoch.
    
    \item We present an efficient strategy to estimate the benefits of the possible triples (i.e., object-predicate-function triple) to compare between them, by leveraging different properties of such triples (i.e., output of previous functions, cost and quality of remaining functions etc.).
    
    
    
    \item We experimentally evaluated our approach using real datasets and tagging functions in different domains (i.e., tweets and images) and demonstrate the efficiency of our approach.
    %\item We propose an approach to progressive processing of queries with predicates that involve tags over untagged datasets.
    
    % \item We present an algorithm to generate execution plans including triples object-predicate-function (i.e., which predicate of which object has to be evaluated with which tagging function) that should be run in order to maximize the quality of the answer of the query.
    
    %\item We present an algorithm to generate execution plans in each epoch that consists of a set of object-predicate-function triples(i.e., which object should be evaluated and with which  tagging function of a predicate) that have the highest potential to improve the quality of the answer set in that epoch.
    
    %\item We present a mechanism to estimate the benefit of a possible triple object-predicate-function using information extracted about the cost and quality of the different functions.%\hl{Remember to add some sneak peek of the results.}

\end{itemize}

The rest of the paper is organized as follows. 
In Section~\ref{sect:problemDefinition}, we define the notation and problem.
In Section~\ref{sect:overview}, we present an overview of the approach.
In Section~\ref{sect:plan generation}, we detail our mechanism to generate and execute plans which has the highest capability of improving the quality of the answer set in each epoch.
In Section~\ref{sect:extensions}, we introduce some extensions to our approach.
In Section~\ref{sect:experiments}, we show the experimental evaluation performed to validate our approach.
Finally, Section~\ref{sect:relatedWork} surveys related works and Section~\ref{sect:conclusions} presents conclusions and future work.
\end{comment}  


==> Motivation.tex <==
\section{Motivation}
We are living in the era of Internet of Things(IoT) where billions of devices are communicating with each other for the purpose of smart applications, smart surveillance, smart monitoring systems. Such systems and applications have given rise to several new types of data processing challenges in big data. Traditional data processing techniques are not well suited for the processing of such an enormous amount of data in near real-time setting. Furthermore, popular data processing techniques such as machine learning techniques, computer vision techniques have become so advanced that they are at the heart of any data processing systems. In this paper, we are addressing the problem of efficient processing of the data using these machine learning techniques in the context of a query.

Lets consider the possible data processing scenarios on such a big data system supporting near-real time latency. One way of processing such large amount of data, can be to store all the data in a central server first and then perform all the processing tasks on the data in an off-line setting. Such an approach will be extremely inefficient, as it will require a long time to finish the processing, then only the system will be able to answer any query. On the other end of the spectrum lies the scenario, where we compute everything at the arrival time of the data in to the system. Suppose the system offers query on ten types of features, we evaluate all these features as soon as the data arrives to the system. All the result of computation is cached in the system and any incoming query is answered using this cached result. This strategy is also extremely inefficient, as it will require us to perform a large amount computation on every data at the arrival time. This will increase the data ingestion time, as well as query processing time for queries on recent data. Further this will require us to cache an arbitrarily large amount of results generated from these functions, which might not be required by any query. 
 
 Our approach lies in between these two end points. Our objective is not to burden the system with unnecessary machine learning tasks and perform analysis only with the context of a query. The goal is to generate a result using the available machine learning techniques and return the result within the query budget specified by the user. 

\subsection{Multimedia Domain}

Automatic multimedia tagging~\cite{MultimediaMotivation}, defined as the process that automatically assigns a set of tags to multimedia data without any interference from humans, is a popular challenge in the multimedia domain. Automatically tagging multimedia content can be beneficial to many tasks such as \hl{TO COMPLETE}. Typically, machine learning techniques are employed to accomplish the tagging by mapping low-level features of multimedia content to semantic tags. For instance, many different approaches have been presented to detect faces~\cite{??,??}, gender~\cite{??,??}, or different objects~\cite{??,??} from images.

Let us consider the Boston marathon bombing, that took place in 2013, as an example of scenario that can benefit from automatic multimedia tagging techniques. Moments after the bombing the authorities had little information about the suspects who were on the run. Indeed, in reality the pervasiveness of cameras in our society (e.g., CCTV in the streets and people carrying their smartphones) helped authorities catch the bombers\footnote{\url{https://www.geekwire.com/2013/security-cameras-helped-catch-boston-marathon-bombers-public-surveillance/}}. The process to analyze camera feeds was performed manually but one can imagine how automatic tagging of content could help in this situation. Ideally, moments after the incident authorities could gather hundreds of thousands of images  from videocameras in the area. Then, they could run a query over such dataset trying to obtain those images containing the potential perpetrator so that forensics can focus on a smaller set of images. For that, they would like to retrieve all the images that match the description of several suspicious people being reported by people in the area (e.g., a male wearing a black backpack and glasses). The following SQL-like query capture such requirements:

\begin{small}
\begin{lstlisting}[mathescape = true,label={lst:QueryExampleImage}]
  SELECT * FROM ImageSet
  WHERE $GenderDetector$(ImageSet.image) = male
  AND $GlassDetector$(ImageSet.image) = true
  AND $BackpackDetector$(ImageSet.image) = true
\end{lstlisting}
\end{small}

Notice that, in this scenario, and specially right after the event, retrieving results fast is incredibly important. However, extraction of such high-level features is sometimes costly. Also, obtaining accurate results would be important but some of these feature extractors work well in different situations (e.g., depending on the light on the image). Hence, several algorithms might have to be run for each feature in order to decrease the uncertainty. 


\subsection{Twitter Domain}

Analysis on Twitter data has attracted great attention in the research community. For instance, twitter data has been used for \hl{X}~\cite{??} and \hl{Y}~\cite{??}. To accomplish such tasks, tweets (sometimes containing images, videos, or URLs in addition to the text) have to be processed to extract higher-level features. There are several types of popular analysis tasks performed on tweets in the literature and many different algorithms to achieve them. For example, sentiment analysis~\cite{TweetSentimentAnalysis1,TweetSentimentAnalysis2,TweetSentimentAnalysis3}, topic analysis~\cite{??,??}, or opinion mining~\cite{??,??}. \hl{Add a couple of references per task} 

As a use case, lets consider the event of the 2016 presidential debate between Hillary Clinton and Donald Trump. Nowadays, newspapers report such events in real-time on their online versions by analyzing each comment made by the participants. Suppose a news paper journalist covering the debate who wants to distinguish their analysis from others. For that, this journalist wants to report in real-time on the general feeling of the public about the proposals of the candidates. Let's imagine that for each 15 minutes segment of the debate (i.e., foreign policy, education, etc.) the reporter gathers tweets to analyze (for instance using the tool presented in~\cite{7930084} \hl{Include reference to Abdul's demo paper}). The reporter would like to pose a query to retrieve tweets with both a positive and negative sentiment about the two candidates. For instance, the following SQL-like query could be used to retrieve tweets about the foreign policy proposals of the candidate Donald Trump:

\begin{small}
\begin{lstlisting}[mathescape = true,label={lst:QueryExampleTweet}]
  SELECT * FROM Tweets
  WHERE $LocationDetector$(Tweets.tweet) = "USA"
  AND $TopicDetector$(Tweets.tweet) = 
      "presidential debate"
  AND $SentimentDetector$(Tweets.tweet) = "positive"
  AND $EntityDetector$(Tweets.tweet, 
      "Donald Trump") = true
  AND $EntityDetector$(Tweets.tweet,
      "Foreign policy") = true
\end{lstlisting}
\end{small}
  
Notice that, due to the need to report the debate in real-time, the reporter would like to retrieve results as fast as possible before going into the next segment. Also, notice that there were 17.1 million interactions on Twitter about the event, according to Nielsen's Social Content Ratings\footnote{\url{https://www.hollywoodreporter.com/news/first-presidential-debate-breaks-twitter-932779}}. Therefore, the challenge is how to execute such query, that needs to extract different features per tweet, for such a large dataset and in near real-time.


\subsection{Internet Of Things Domain}

The Internet Of Things (IoT)~\cite{Atzori:2010:ITS:1862461.1862541}, where devices are interconnected enabling them to exchange date, can benefit a large number of scenarios. For instance, the IoT will enable the development of \emph{smart cities} where parking spaces, urban noise, traffic congestion, street lighting, irrigation, and waste can be monitored in real time and managed more effectively. There is a need of efficient techniques to analyze and process IoT sensor data to enable such smart services. In fact, approaches have been presented in the literature to \hl{TODO: include some examples of possible classifiers that have been proposed in the context of the IoT.}

%IoT applications fall into two general categories~\cite{7582463}: 1) ambient data collection and analytics and 2) real-time reactive applications. The first category of applications generally involves collecting sensor data from a variety of sensors (e.g., wearable devices), process them offline to gain actionable information (e.g., a model) and then run the model as a predictor for new data collected from the sensor in the future. The second category of applications involves real-time reactive systems such as autonomous vehicle or manufacturing processes where the systems make real-time decisions based on observed sensor values. 

Lets consider a smart building as an example of IoT scenario and one of the most important tasks in building management: controlling of the Heating, Ventilation and Air-conditioning (HVAC) unit of the building. Nowadays, buildings typically implement a range of temperatures for the different rooms depending on whether the room is occupied or not. With IoT sensors within the building, this task could be further advance in order to provide \emph{personalized thermal comfort}~\cite{??} for the inhabitants of the building. For instance, the temperature in offices or meeting rooms could be adapted to the preferences of the people in them. To enable this personalized-thermal comfort the smart building should then determine several features for each room: who is inside and what is the activity taking place in it. This information could be inferred from sensor data in the building. For instance, to determine the activity microphones~\cite{??} or cameras~\cite{??} can be used and to determine who is inside using WiFi access point sensors, beacon sensors, mobile phone sensors, motion sensors etc. In this case, the building management system would want to pose the following query:

\begin{small}
\begin{lstlisting}[mathescape = true,label={lst:QueryExampleHvac}]
SELECT $OccupancyDetectorWifi$(SELECT * FROM
Observations where type = "WifiAP" AND 
timeStamp > "2017-08-28 16:10:09" 
AND  timeStamp < "2017-08-28 16:15:09"),

$OccupancyDetectorBeacon$(SELECT * 
FROM Observations where type = 
"Beacon" AND 
timeStamp > "2017-08-28 16:10:09" 
AND  timeStamp < "2017-08-28 16:15:09"),

$OccupancyDetectorMotion$(SELECT * 
FROM Observations where type = 
"Motion" AND 
timeStamp > "2017-08-28 16:10:09" 
AND  timeStamp < "2017-08-28 16:15:09")
\end{lstlisting}  
\end{small}

Imagine that the occupancy level inside the rooms are very dynamic in nature, i.e., it changes every five minutes. It is impossible for the BMS to analyze all these data every five minutes and produce accurate occupancy of all the rooms inside the building. In such a scenario, the BMS can pose the following SQL query to the system: 

The query budget in this case can be five minutes. This query determines the occupancy of each room in side a building using three functions $OccupancyDetectorWifi$, \\  $OccupancyDetectorBeacon$, $OccupancyDetectorMotion$. In this scenario, the system will be executing these functions in such a way so that it can return the answer set within five minutes. 

==> ObjectSelection.tex <==
\section{Object selection }\label{sec:object selection}
In the previous section, we have derived the strategy to choose an answer set that will maximize the $F_1$ measure of an answer set.In this section we will explore the criteria of selecting an $(object,classifier)$ pair based on expected quality improvement. For every objects in the dataset, we define a state of the object.

%\textbf{State of an object:} State of an object represents the execution algorithms that have already been executed on the object. E.g an object might have passed through three classifiers $c_1$, $c_2$, and $c_3$, then the state of object is $s_{123}$. 

Given a state where the objects have probabilities $p_1$,$p_2$, $p_3$...$p_N$, we will determine which is the best $(object,classifier)$ pair to be executed in the next iteration. Suppose the current answer set contains objects with probabilities $p_1$,$p_2$, $p_3$.. $p_n$. For each of the objects outside of the answer set we calculate $benefit$ values. Benefit value is defined as amount of $F_1$ measure improvement per unit cost. 
\begin{equation}\label{eqn:benefit}
Benefit(o_i) = \frac{\Delta F_1}{\Delta cost}
\end{equation}
where, $\Delta F_1$ measures the amount of $F_1$ measure improvement if we execute the next algorithm and $\Delta cost$ is time required to execute the next algorithm.

\subsection{Naive Approach:} One naive way to choose a $(classifier,object)$ pair, is to calculate $F_1$ measure improvement for all the objects in the answer set. For calculating $F_1$ measure of an object, we first perform threshold selection algorithm. After threshold is determined, we calculate new $F_1$ measure of the answer set and determine improvement in $F_1$ measure from the previous state.Note that, we compare this new state for a single object only and we assume that remaining all the objects are remaining in the previous state. i.e. suppose we are deciding on object $o_5$. Then we consider the probability values in new state as $p_1$,$p_2$, ...$p_5'$ ,...$p_N$, i.e. only probability value of $o_5$ is changed, remaining values are same. In this state we calculate $F_1$ measure of the answer set and determine the improvement from current $F_1$ measure of the answer set. For each of the objects, we determine improvement in $F_1$ measure and calculate $benefit$ according to equation \ref{eqn:benefit}. After the calculation of benefit values, we rank the objects based on their benefit values and choose the object with maximum benefit value. Next, in the execution phase, we execute the $execution algorithm$ on the object and calculate new $F_1$ measure of answer set. After this step, we reiterate the process of benefit calculation and decide which object should be chosen for next execution round.   

\subsection{Heuristic Approach} In Naive Approach, we have seen that we have to perform threshold selection algorithm every time probability of an object is updated. Furthermore, we were calculating benefit of all the objects, including the objects in the answer set, which is a very high overhead. In this part, we try to establish a condition, which will reduce the number of execution of threshold selection algorithm. As seen in Equation \ref{eqn:benefit}, $benefit$ calculation is dependent on $F_1$ measure calculation, and $F_1$ measure calculation can be done only when we perform threshold selection algorithm first. But in this section, we try to establish a relation, where $benefit$ calculation is not dependent on this threshold selection step, rather it is dependent on local property of the object, i.e., it's current probability, change in probability etc.

\begin{definition}
Let's consider two objects with probabilities $p_i$ and $p_j$ where $p_i > p_j$, and corresponding increment in probability values as $\Delta p_i$ and $\Delta p_j$, and the $\Delta cost$ value for both the objects are same.Suppose both the new probability values i.e. $(p_1+ \Delta p_1)$ and $(p_2+ \Delta p_2)$  are greater than current threshold probability $p_\tau$. Then object $o_i$ will increase $F_1$ measure more compared to $o_j$ if the following conditions holds:
\begin{enumerate}
\item $  p_1(p_1+ \Delta p_1) > p_2(p_2+\Delta p_2) $
\end{enumerate}
\end{definition}


\begin{proof}
Suppose the current threshold probability is $p_m$, and current $F_1$ measure is $\frac{2(p_1+...p_m)}{p_1+p_2..p_n+ m}$. Let us denote the numerator as $X$ and the value $(p_1+p_2..p_n+ m +1)$ as $Y$. Now if we include object $o_i$ in the answer set, then the numerator becomes $X+p_i+\Delta p_i$ and denominator becomes $Y+\Delta p_i$. So the new $F_1$ measure will be $\frac{X+p_i+\Delta p_i}{Y+\Delta p_i}$. Similarly $F_1$ measure of the answer set if we include object $o_j$ will be $\frac{X+p_j+\Delta p_j}{Y+\Delta p_j}$. Now if $F_1$ measure of object $o_i$ is more than $o_j$ then object $o_i$ will have more benefit value. We solve the following inequality:
\begin{equation}\label{eqn:DeriveBenefitCondition}
\begin{split}
&p_i\frac{X+p_i+\Delta p_i}{Y+\Delta p_i} > p_j\frac{X+p_j+\Delta p_j}{Y+\Delta p_j}\\
& \Rightarrow (p_iX + p_i\Delta p_i+p_i^2)(Y+\Delta p_j) > (p_jX+p_j^2+pj\Delta p_j)(Y+\Delta p_i) \\
& \Rightarrow (p_i-p_j)XY + Y(p_i\Delta p_i+p_i^2-p_j^2-p_j\Delta p_j) \\
	&+ X(p_i\Delta p_j-p_j \Delta p_i) + (\Delta p_i \Delta p_j(p_i-p_j) + p_i^2\Delta p_j - p_j^2\Delta p_i) >0 \\ 
& \Rightarrow Q_1 + Q_2 + Q_3 + Q_4 >0
\end{split}
\end{equation}
The term $Q_1$ is greater than zero as $p_i>p_j$. Lets consider that increment $\Delta p_i < \Delta p_j$. Then  coefficient of $X$ will be greater than zero, which implies the term $Q_3$ is more than 0. Similarly the term $Q_4$ will also be greater than zero. So the only term that can be negative is $Q_2$. If the coefficient of $Y$ becomes positive, then the  inequality $Q_1+ Q_2+Q_3+Q_4 > 0$ holds. Simplifying the coefficient of Y, we get the condition as follows: 
\begin{equation}
p_i(p_i+\Delta p_i) > p_j(p_j+ \Delta p_j)
\end{equation}
\end{proof}

Lets consider the scenario, where $\Delta cost$ value of the two objects are not same.  Let us denote the value of $\frac{p_i}{\Delta cost_i}$ as $\nu_i$, and similarly, the value of $\frac{p_j}{\Delta cost_j}$ as  $\nu_j$

\begin{definition} \label{lemma:SelectionCriteria}
Let's consider two objects with probabilities $p_i$ and $p_j$ where $p_i > p_j$, and corresponding increment in probability values as $\Delta p_i$ and $\Delta p_j$.Then object $o_i$ will have more $benefit$ value compared to object $o_j$ if the following conditions hold:
\begin{enumerate}
\item $ \nu_1(p_1+ \Delta p_1) > \nu_2(p_2+\Delta p_2)$ 
\end{enumerate}
\end{definition}

\begin{proof}
If we follow the similar kind of equation as equation \ref{eqn:DeriveBenefitCondition}, then the first line of the equation becomes $\nu_i\frac{X+p_i+\Delta p_i}{Y+\Delta p_i} > \nu_j\frac{X+p_j+\Delta p_j}{Y+\Delta p_j}$. Finally considering the coefficient of Y in line 3 in equation \ref{eqn:DeriveBenefitCondition}, we get the following condition for choosing object $o_i$ over $o_j$:
\begin{equation}
\nu_i(p_i+\Delta p_i) > \nu_j(p_j+ \Delta p_j)
\end{equation}
\end{proof}

In this heuristic approach, we always consider the objects which are currently not in the answer set. Among the objects, which are currently not in the answer set, we order them based on the metric derived in lemma \ref{lemma:SelectionCriteria}. From these objects we choose top $k$ objects for the execution in the next round. In the next round, we execute these $k$ objects and calculate new threshold probability of the answer set. We keep iterating this process until the time budget is finished.
%Complexity arises when we perform this threshold selection algorithm \ref{algo:ThresholdSelection}. In this section, we want to establish a criteria, through which we do not have to perform threshold selection algorithm \ref{algo:ThresholdSelection}, for calculating benefit of an object.

\textbf{Choosing an appropriate block size k:}
As explained in the previous section, we order the objects and execution algorithms based on their benefit values. Among these objects we choose $k$ objects to be executed in the next iteration. For determining appropriate value of $k$, we consider an approach based on time. As seen in the algorithm, \ref{fig:Choose Next Best}, we first decide which is the next best classifier for each objects outside of the answer set. Then we determine the benefit of each of these objects. Finding the next best classifier and calculating benefit, is looking up from an appropriate list first and  then calculation of benefit value is done according to lemma \ref{lemma:SelectionCriteria}. Cost of these two steps is constant for every objects outside of the answer set and lets denote it by $t_0$. Suppose the dataset contains $N$ objects and the current answer set contains $\tau$ objects, then we have to calculate benefit of $N-\tau$ objects. Suppose cost of running the threshold selection algorithm where the probability of only one object is changed, is $k_1$ and running the same algorithm where probability $k$ objects changed is $k_1+ k \Delta$.Suppose average runtime of a classifier is $c1$. 
Let us consider two scenarios, where we execute only one $(object,classifier)$ pair in the execution phase vs where we run $k$  ($object$,$cassifier$) pairs. So in approach 1, the amount of time taken in one iteration is $(N-\tau)t_0 + k_1+c_1$. In approach 2, the amount of time taken is $(N-\tau)t_0 + (k_1+k\Delta)+kc_1$, since threshold selection cost  and execution cost increased. Suppose the query budget is $B$, then number of iteration possible in first approach is $\frac{B}{(N-\tau)t_0 + k_1+c_1}$ and in second approach the number of iteration is $\frac{B}{(N-\tau)t_0 + (k_1+k\Delta)+kc_1}$. If we consider the time spent in the execution phase, as $effective time$,then $effective time$ in approach 2 should be more than $effective time$ in approach 2. Based on this inequality, we derive the following condition:
\begin{equation}\label{eqn:selectionk}
\begin{split}
&\frac{B}{(N-\tau)t_0 + (k_1+k\Delta)+kc_1} kc_1 > \frac{B}{(N-\tau)t_0 + k_1+c_1} c_1 \\
& \Rightarrow k((N-\tau)t_0 + k_1+c_1) > ((N-\tau)t_0 + (k_1+k\Delta)+kc_1) \\
& \Rightarrow k > \frac{(N-\tau)t_0 + k_1}{(N-\tau)t_0 + k_1-\Delta}
\end{split}
\end{equation}

Based on the above equation \ref{eqn:selectionk} we choose the value of k to be $\frac{(N-\tau)t_0 + k_1}{(N-\tau)t_0 + k_1-\Delta}$, where $\tau$ is the size of current answer set, $t_0$ is the cost of benefit calculation for one object.

However if $\Delta$ value is negligible, then it implies that the decision making time is constant in every iterations. In that scenario, we allocate certain percentage of the query budget for the purpose of decision making. E.g. suppose 10 \% of the query budget $B$ is allocated for decision making process. So in the entire query execution process, $0.1B$ amount of time will be spent in decision making and $0.9B$ amount of time will be spent in execution process. Suppose, it takes $t_1$ seconds for decision making in one iteration, then number of iterations will be $\frac{0.1B}{t_1}$ and in every iteration $9t_1$ seconds will be spent in the execution process. So the value of $k$ in this scenario will be $\frac{9t_1}{c_1}$.
